Observation of Entanglement Enabled Spin-Interference in the Drell-S\"oding Process in Au+Au Ultraperipheral Collisions at RHIC

We report a measurement of the Drell-S\"oding $\pi^+ \pi^-$ production in Au + Au ultraperipheral collisions at a center-of-mass energy per nucleon pair $\sqrt{s_{NN}} = 200~\mathrm{GeV}$ using the STAR detector. For the first time, the Entanglement Enabled Spin-Interference (EESI) effect is observed in the Drell-S\"oding process through the amplitude $A_{2\Delta\phi}$ of the $\cos(2\Delta\phi)$ modulation. The measured $A_{2\Delta\phi}$ exhibits no significant dependence on the invariant mass $M_{\pi^+ \pi^-}$. An enhancement of three standard deviations is observed for the Drell-S\"oding process compared to $\rho^0$ photoproduction. Furthermore, we measure the $|t|$-dependence of the Drell-S\"oding process and $\rho^0$ photoproduction. The Drell-S\"oding spectrum falls more steeply with $|t|$ and exhibits diffractive structures shifted to lower $|t|$ compared to $\rho^0$ photoproduction, features that are not captured by theoretical calculations. These results provide new insights into the interplay between quantum interference and photon-nuclear interactions in ultra-peripheral heavy-ion collisions.

==> acknowledgement.tex <==
\section*{Acknowledgement}

We thank the RHIC Operations Group and SDCC at BNL, the NERSC Center at LBNL, and the Open Science Grid consortium for providing resources and support.  This work was supported in part by the Office of Nuclear Physics within the U.S. DOE Office of Science, the U.S. National Science Foundation, National Natural Science Foundation of China, Chinese Academy of Science, the Ministry of Science and Technology of China and the Chinese Ministry of Education, NSTC Taipei, the National Research Foundation of Korea, Czech Science Foundation and Ministry of Education, Youth and Sports of the Czech Republic, Hungarian National Research, Development and Innovation Office, New National Excellency Programme of the Hungarian Ministry of Human Capacities, Department of Atomic Energy and Department of Science and Technology of the Government of India, the National Science Centre and WUT ID-UB of Poland, German Bundesministerium f\"ur Bildung, Wissenschaft, Forschung and Technologie (BMBF), Helmholtz Association, Ministry of Education, Culture, Sports, Science, and Technology (MEXT), and Japan Society for the Promotion of Science (JSPS).

==> authorlistB.tex <==
\affiliation{Academia Sinica}
\affiliation{Abilene Christian University, Abilene, Texas   79699}
\affiliation{AGH University of Krakow, FPACS, Cracow 30-059, Poland}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\affiliation{American University in Cairo, New Cairo 11835, Egypt}
\affiliation{Ball State University, Muncie, Indiana, 47306}
\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\affiliation{University of Calabria \& INFN-Cosenza, Rende 87036, Italy}
\affiliation{University of California, Berkeley, California 94720}
\affiliation{University of California, Davis, California 95616}
\affiliation{University of California, Los Angeles, California 90095}
\affiliation{University of California, Riverside, California 92521}
\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\affiliation{Chongqing University, Chongqing, 401331}
\affiliation{Creighton University, Omaha, Nebraska 68178}
\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\affiliation{Technische Universit\"at Darmstadt, Darmstadt 64289, Germany}
\affiliation{National Institute of Technology Durgapur, Durgapur - 713209, India}
\affiliation{ELTE E\"otv\"os Lor\'and University, Budapest, Hungary H-1117}
\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\affiliation{Fudan University, Shanghai, 200433 }
\affiliation{Guangxi Normal University, Guilin, 541004}
\affiliation{University of Heidelberg, Heidelberg 69120, Germany }
\affiliation{University of Houston, Houston, Texas 77204}
\affiliation{Huzhou University, Huzhou, Zhejiang  313000}
\affiliation{Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\affiliation{Indian Institute Technology, Patna, Bihar 801106, India}
\affiliation{Indiana University, Bloomington, Indiana 47408}
\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\affiliation{University of Jammu, Jammu 180001, India}
\affiliation{Kent State University, Kent, Ohio 44242}
\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\affiliation{Lanzhou University}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\affiliation{Max-Planck-Institut f\"ur Physik, Munich 80805, Germany}
\affiliation{Michigan State University, East Lansing, Michigan 48824}
\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\affiliation{National Cheng Kung University, Tainan 70101 }
\affiliation{Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}
\affiliation{The Ohio State University, Columbus, Ohio 43210}
\affiliation{Panjab University, Chandigarh 160014, India}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\affiliation{Rice University, Houston, Texas 77251}
\affiliation{Rutgers University, Piscataway, New Jersey 08854}
\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\affiliation{South China Normal University, Guangzhou, Guangdong 510631}
\affiliation{Sejong University, Seoul, 05006, South Korea}
\affiliation{Shandong University, Qingdao, Shandong 266237}
\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\affiliation{Southern Connecticut State University, New Haven, Connecticut 06515}
\affiliation{State University of New York, Stony Brook, New York 11794}
\affiliation{Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Arica 1000000, Chile}
\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\affiliation{University of Texas, Austin, Texas 78712}
\affiliation{Tsinghua University, Beijing 100084}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\affiliation{University of Chinese Academy of Sciences, Beijing, 101408}
\affiliation{United States Naval Academy, Annapolis, Maryland 21402}
\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\affiliation{Wayne State University, Detroit, Michigan 48201}
\affiliation{Wuhan University of Science and Technology, Wuhan, Hubei 430065}
\affiliation{Yale University, New Haven, Connecticut 06520}

\author{B.~E.~Aboona}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{J.~Adam}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{L.~Adamczyk}\affiliation{AGH University of Krakow, FPACS, Cracow 30-059, Poland}
\author{I.~Aggarwal}\affiliation{Panjab University, Chandigarh 160014, India}
\author{M.~M.~Aggarwal}\affiliation{Panjab University, Chandigarh 160014, India}
\author{Z.~Ahammed}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{E.~C.~Aschenauer}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~Aslam}\affiliation{Indian Institute Technology, Patna, Bihar 801106, India}
\author{J.~Atchison}\affiliation{Abilene Christian University, Abilene, Texas   79699}
\author{V.~Bairathi}\affiliation{Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Arica 1000000, Chile}
\author{X.~Bao}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{K.~Barish}\affiliation{University of California, Riverside, California 92521}
\author{S.~Behera}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{R.~Bellwied}\affiliation{University of Houston, Houston, Texas 77204}
\author{P.~Bhagat}\affiliation{University of Jammu, Jammu 180001, India}
\author{A.~Bhasin}\affiliation{University of Jammu, Jammu 180001, India}
\author{S.~Bhatta}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{S.~R.~Bhosale}\affiliation{AGH University of Krakow, FPACS, Cracow 30-059, Poland}
\author{J.~Bielcik}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{J.~Bielcikova}\affiliation{Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}
\author{J.~D.~Brandenburg}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{C.~Broodo}\affiliation{University of Houston, Houston, Texas 77204}
\author{X.~Z.~Cai}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{H.~Caines}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Calder{\'o}n~de~la~Barca~S{\'a}nchez}\affiliation{University of California, Davis, California 95616}
\author{D.~Cebra}\affiliation{University of California, Davis, California 95616}
\author{J.~Ceska}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{I.~Chakaberia}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{P.~Chaloupka}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{B.~K.~Chan}\affiliation{University of California, Los Angeles, California 90095}
\author{Z.~Chang}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{A.~Chatterjee}\affiliation{National Institute of Technology Durgapur, Durgapur - 713209, India}
\author{D.~Chen}\affiliation{University of California, Riverside, California 92521}
\author{J.~Chen}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{J.~H.~Chen}\affiliation{Fudan University, Shanghai, 200433 }
\author{Q.~Chen}\affiliation{Guangxi Normal University, Guilin, 541004}
\author{Z.~Chen}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{J.~Cheng}\affiliation{Tsinghua University, Beijing 100084}
\author{Y.~Cheng}\affiliation{University of California, Los Angeles, California 90095}
\author{W.~Christie}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{X.~Chu}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~Corey}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{H.~J.~Crawford}\affiliation{University of California, Berkeley, California 94720}
\author{M.~Csan\'{a}d}\affiliation{ELTE E\"otv\"os Lor\'and University, Budapest, Hungary H-1117}
\author{G.~Dale-Gau}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{A.~Das}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{I.~M.~Deppner}\affiliation{University of Heidelberg, Heidelberg 69120, Germany }
\author{A.~Deshpande}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{A.~Dhamija}\affiliation{Panjab University, Chandigarh 160014, India}
\author{A.~Dimri}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{P.~Dixit}\affiliation{Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\author{X.~Dong}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~L.~Drachenberg}\affiliation{Abilene Christian University, Abilene, Texas   79699}
\author{E.~Duckworth}\affiliation{Kent State University, Kent, Ohio 44242}
\author{J.~C.~Dunlop}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{J.~Engelage}\affiliation{University of California, Berkeley, California 94720}
\author{G.~Eppley}\affiliation{Rice University, Houston, Texas 77251}
\author{S.~Esumi}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{O.~Evdokimov}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{O.~Eyser}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{R.~Fatemi}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{S.~Fazio}\affiliation{University of Calabria \& INFN-Cosenza, Rende 87036, Italy}
\author{Y.~Feng}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{E.~Finch}\affiliation{Southern Connecticut State University, New Haven, Connecticut 06515}
\author{Y.~Fisyak}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{F.~A.~Flor}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{C.~Fu}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{T.~Fu}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{C.~A.~Gagliardi}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{T.~Galatyuk}\affiliation{Technische Universit\"at Darmstadt, Darmstadt 64289, Germany}
\author{T.~Gao}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{F.~Geurts}\affiliation{Rice University, Houston, Texas 77251}
\author{N.~Ghimire}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{A.~Gibson}\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\author{K.~Gopal}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{X.~Gou}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{D.~Grosnick}\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\author{A.~Gu}\affiliation{Huzhou University, Huzhou, Zhejiang  313000}
\author{A.~Gupta}\affiliation{University of Jammu, Jammu 180001, India}
\author{A.~Hamed}\affiliation{American University in Cairo, New Cairo 11835, Egypt}
\author{X.~Han}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{S.~Harabasz}\affiliation{Technische Universit\"at Darmstadt, Darmstadt 64289, Germany}
\author{M.~D.~Harasty}\affiliation{University of California, Davis, California 95616}
\author{J.~W.~Harris}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{H.~Harrison-Smith}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{L.~B.~ Havener}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{X.~H.~He}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{Y.~He}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{N.~Herrmann}\affiliation{University of Heidelberg, Heidelberg 69120, Germany }
\author{L.~Holub}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{C.~Hu}\affiliation{University of Chinese Academy of Sciences, Beijing, 101408}
\author{Q.~Hu}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{Y.~Hu}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{H.~Huang}\affiliation{National Cheng Kung University, Tainan 70101 }
\author{H.~Z.~Huang}\affiliation{University of California, Los Angeles, California 90095}
\author{S.~L.~Huang}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{T.~Huang}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{Y.~Huang}\affiliation{Tsinghua University, Beijing 100084}
\author{Y.~Huang}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{T.~J.~Humanic}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{M.~Isshiki}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{W.~W.~Jacobs}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{A.~Jalotra}\affiliation{University of Jammu, Jammu 180001, India}
\author{C.~Jena}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{A.~Jentsch}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Y.~Ji}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~Jia}\affiliation{State University of New York, Stony Brook, New York 11794}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{C.~Jin}\affiliation{Rice University, Houston, Texas 77251}
\author{N.~ Jindal}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{X.~Ju}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{E.~G.~Judd}\affiliation{University of California, Berkeley, California 94720}
\author{S.~Kabana}\affiliation{Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Arica 1000000, Chile}
\author{D.~Kalinkin}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{K.~Kang}\affiliation{Tsinghua University, Beijing 100084}
\author{D.~Kapukchyan}\affiliation{University of California, Riverside, California 92521}
\author{K.~Kauder}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{D.~Keane}\affiliation{Kent State University, Kent, Ohio 44242}
\author{A.~ Khanal}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{Y.~V.~Khyzhniak}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{D.~P.~Kiko\l{}a~}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{J.~Kim}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{D.~Kincses}\affiliation{ELTE E\"otv\"os Lor\'and University, Budapest, Hungary H-1117}
\author{I.~Kisel}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\author{A.~Kiselev}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{A.~G.~Knospe}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{H.~S.~Ko}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~Ko{\l}a\'s}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{B.~Korodi}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{L.~K.~Kosarzewski}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{L.~Kumar}\affiliation{Panjab University, Chandigarh 160014, India}
\author{M.~C.~Labonte}\affiliation{University of California, Davis, California 95616}
\author{R.~Lacey}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{J.~M.~Landgraf}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{C.~ Larson}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{J.~Lauret}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{A.~Lebedev}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{J.~H.~Lee}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Y.~H.~Leung}\affiliation{University of Heidelberg, Heidelberg 69120, Germany }
\author{C.~Li}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{D.~Li}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{H-S.~Li}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{H.~Li}\affiliation{Wuhan University of Science and Technology, Wuhan, Hubei 430065}
\author{H.~Li}\affiliation{Guangxi Normal University, Guilin, 541004}
\author{W.~Li}\affiliation{Rice University, Houston, Texas 77251}
\author{X.~Li}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{X.~Li}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{Y.~Li}\affiliation{Tsinghua University, Beijing 100084}
\author{Z.~Li}\affiliation{South China Normal University, Guangzhou, Guangdong 510631}
\author{Z.~Li}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{X.~Liang}\affiliation{University of California, Riverside, California 92521}
\author{Y.~Liang}\affiliation{Kent State University, Kent, Ohio 44242}
\author{R.~Licenik}\affiliation{Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{T.~Lin}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Y.~Lin}\affiliation{Guangxi Normal University, Guilin, 541004}
\author{M.~A.~Lisa}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{C.~Liu}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{G.~Liu}\affiliation{South China Normal University, Guangzhou, Guangdong 510631}
\author{H.~Liu}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{L.~Liu}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{Z.~Liu}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{T.~Ljubicic}\affiliation{Rice University, Houston, Texas 77251}
\author{O.~Lomicky}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{R.~S.~Longacre}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{E.~M.~Loyd}\affiliation{University of California, Riverside, California 92521}
\author{T.~Lu}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{J.~Luo}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{X.~F.~Luo}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{L.~Ma}\affiliation{Fudan University, Shanghai, 200433 }
\author{R.~Ma}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Y.~G.~Ma}\affiliation{Fudan University, Shanghai, 200433 }
\author{D.~Mallick}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{R.~Manikandhan}\affiliation{University of Houston, Houston, Texas 77204}
\author{S.~Margetis}\affiliation{Kent State University, Kent, Ohio 44242}
\author{C.~Markert}\affiliation{University of Texas, Austin, Texas 78712}
\author{O.~Matonoha}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{O.~Mezhanska}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{K.~Mi}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{S.~Mioduszewski}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{B.~Mohanty}\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\author{B.~Mondal}\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\author{M.~M.~Mondal}\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\author{I.~Mooney}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{J.~Mrazkova}\affiliation{Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{M.~I.~Nagy}\affiliation{ELTE E\"otv\"os Lor\'and University, Budapest, Hungary H-1117}
\author{C.~J.~Naim}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{A.~S.~Nain}\affiliation{Panjab University, Chandigarh 160014, India}
\author{J.~D.~Nam}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{M.~Nasim}\affiliation{Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\author{H.~Nasrulloh}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{D.~Neff}\affiliation{University of California, Los Angeles, California 90095}
\author{J.~M.~Nelson}\affiliation{University of California, Berkeley, California 94720}
\author{M.~Nie}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{G.~Nigmatkulov}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{T.~Niida}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{T.~Nonaka}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{G.~Odyniec}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{A.~Ogawa}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~Oh}\affiliation{Sejong University, Seoul, 05006, South Korea}
\author{K.~Okubo}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{B.~S.~Page}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~Pal}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{A.~Pandav}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{A.~Panday}\affiliation{Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\author{A.~K.~Pandey}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{T.~Pani}\affiliation{Rutgers University, Piscataway, New Jersey 08854}
\author{A.~Paul}\affiliation{University of California, Riverside, California 92521}
\author{S.~Paul}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{D.~Pawlowska}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{C.~Perkins}\affiliation{University of California, Berkeley, California 94720}
\author{J.~Pluta}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{B.~R.~Pokhrel}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{I.~D.~ Ponce~Pinto}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Posik}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{S.~Prodhan}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{T.~L.~Protzman}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{A.~Prozorov}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{V.~Prozorova}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{N.~K.~Pruthi}\affiliation{Panjab University, Chandigarh 160014, India}
\author{M.~Przybycien}\affiliation{AGH University of Krakow, FPACS, Cracow 30-059, Poland}
\author{J.~Putschke}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{Z.~Qin}\affiliation{Tsinghua University, Beijing 100084}
\author{H.~Qiu}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{S.~K.~Radhakrishnan}\affiliation{Kent State University, Kent, Ohio 44242}
\author{A.~Rana}\affiliation{Panjab University, Chandigarh 160014, India}
\author{R.~L.~Ray}\affiliation{University of Texas, Austin, Texas 78712}
\author{R.~Reed}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{C.~W.~ Robertson}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{M.~Robotkova}\affiliation{Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{M.~ A.~Rosales~Aguilar}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{D.~Roy}\affiliation{Rutgers University, Piscataway, New Jersey 08854}
\author{P.~Roy~Chowdhury}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{L.~Ruan}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{A.~K.~Sahoo}\affiliation{Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\author{N.~R.~Sahoo}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{H.~Sako}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{S.~Salur}\affiliation{Rutgers University, Piscataway, New Jersey 08854}
\author{S.~S.~Sambyal}\affiliation{University of Jammu, Jammu 180001, India}
\author{J.~K.~Sandhu}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{S.~Sato}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{B.~C.~Schaefer}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{N.~Schmitz}\affiliation{Max-Planck-Institut f\"ur Physik, Munich 80805, Germany}
\author{F-J.~Seck}\affiliation{Technische Universit\"at Darmstadt, Darmstadt 64289, Germany}
\author{J.~Seger}\affiliation{Creighton University, Omaha, Nebraska 68178}
\author{R.~Seto}\affiliation{University of California, Riverside, California 92521}
\author{P.~Seyboth}\affiliation{Max-Planck-Institut f\"ur Physik, Munich 80805, Germany}
\author{N.~Shah}\affiliation{Indian Institute Technology, Patna, Bihar 801106, India}
\author{P.~V.~Shanmuganathan}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{T.~Shao}\affiliation{Fudan University, Shanghai, 200433 }
\author{M.~Sharma}\affiliation{University of Jammu, Jammu 180001, India}
\author{N.~Sharma}\affiliation{Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\author{R.~Sharma}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{S.~R.~ Sharma}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{A.~I.~Sheikh}\affiliation{Kent State University, Kent, Ohio 44242}
\author{D.~Shen}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{D.~Y.~Shen}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{K.~Shen}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{S.~Shi}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{Y.~Shi}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{F.~Si}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{J.~Singh}\affiliation{Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Arica 1000000, Chile}
\author{S.~Singha}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{P.~Sinha}\affiliation{Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\author{M.~J.~Skoby}\affiliation{Ball State University, Muncie, Indiana, 47306}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{N.~Smirnov}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{Y.~S\"{o}hngen}\affiliation{University of Heidelberg, Heidelberg 69120, Germany }
\author{Y.~Song}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{T.~D.~S.~Stanislaus}\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\author{M.~Stefaniak}\affiliation{The Ohio State University, Columbus, Ohio 43210}
\author{Y.~Su}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{M.~Sumbera}\affiliation{Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}
\author{X.~Sun}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{Y.~Sun}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{B.~Surrow}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{M.~Svoboda}\affiliation{Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{Z.~W.~Sweger}\affiliation{University of California, Davis, California 95616}
\author{A.~C.~Tamis}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{A.~H.~Tang}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Z.~Tang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{T.~Tarnowsky}\affiliation{Michigan State University, East Lansing, Michigan 48824}
\author{J.~H.~Thomas}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{A.~R.~Timmins}\affiliation{University of Houston, Houston, Texas 77204}
\author{D.~Tlusty}\affiliation{Creighton University, Omaha, Nebraska 68178}
\author{T.~Todoroki}\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\author{D.~Torres~Valladares}\affiliation{Rice University, Houston, Texas 77251}
\author{S.~Trentalange}\affiliation{University of California, Los Angeles, California 90095}
\author{P.~Tribedy}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~K.~Tripathy}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{T.~Truhlar}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{B.~A.~Trzeciak}\affiliation{Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\author{O.~D.~Tsai}\affiliation{University of California, Los Angeles, California 90095}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{C.~Y.~Tsang}\affiliation{Kent State University, Kent, Ohio 44242}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Z.~Tu}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{J.~Tyler}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{T.~Ullrich}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{D.~G.~Underwood}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\author{G.~Van~Buren}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{J.~Vanek}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{I.~Vassiliev}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\author{F.~Videb{\ae}k}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~A.~Voloshin}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{F.~Wang}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{G.~Wang}\affiliation{University of California, Los Angeles, California 90095}
\author{J.~S.~Wang}\affiliation{Huzhou University, Huzhou, Zhejiang  313000}
\author{J.~Wang}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{K.~Wang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{X.~Wang}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Y.~Wang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{Y.~Wang}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{Y.~Wang}\affiliation{Tsinghua University, Beijing 100084}
\author{Z.~Wang}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{A.~J.~Watroba}\affiliation{AGH University of Krakow, FPACS, Cracow 30-059, Poland}
\author{J.~C.~Webb}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{P.~C.~Weidenkaff}\affiliation{University of Heidelberg, Heidelberg 69120, Germany }
\author{G.~D.~Westfall}\affiliation{Michigan State University, East Lansing, Michigan 48824}
\author{D.~Wielanek}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{H.~Wieman}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{G.~Wilks}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{S.~W.~Wissink}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{R.~Witt}\affiliation{United States Naval Academy, Annapolis, Maryland 21402}
\author{C.~P.~Wong}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{J.~Wu}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{J.~Wu}\affiliation{University of Chinese Academy of Sciences, Beijing, 101408}
\author{X.~Wu}\affiliation{University of California, Los Angeles, California 90095}
\author{X,Wu}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{B.~Xi}\affiliation{Fudan University, Shanghai, 200433 }
\author{Z.~G.~Xiao}\affiliation{Tsinghua University, Beijing 100084}
\author{G.~Xie}\affiliation{University of Chinese Academy of Sciences, Beijing, 101408}
\author{W.~Xie}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{H.~Xu}\affiliation{Huzhou University, Huzhou, Zhejiang  313000}
\author{N.~Xu}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{Q.~H.~Xu}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Y.~Xu}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Y.~Xu}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{Z.~Xu}\affiliation{Kent State University, Kent, Ohio 44242}
\author{Z.~Xu}\affiliation{University of California, Los Angeles, California 90095}
\author{G.~Yan}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Z.~Yan}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{C.~Yang}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Q.~Yang}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{S.~Yang}\affiliation{South China Normal University, Guangzhou, Guangdong 510631}
\author{Y.~Yang}\affiliation{Academia Sinica}\affiliation{National Cheng Kung University, Tainan 70101 }
\author{Z.~Ye}\affiliation{South China Normal University, Guangzhou, Guangdong 510631}
\author{Z.~Ye}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{L.~Yi}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Y.~Yu}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{H.~Zbroszczyk}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{W.~Zha}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{C.~Zhang}\affiliation{Fudan University, Shanghai, 200433 }
\author{D.~Zhang}\affiliation{South China Normal University, Guangzhou, Guangdong 510631}
\author{J.~Zhang}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{S.~Zhang}\affiliation{Chongqing University, Chongqing, 401331}
\author{W.~Zhang}\affiliation{South China Normal University, Guangzhou, Guangdong 510631}
\author{X.~Zhang}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{Y.~Zhang}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\author{Y.~Zhang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{Y.~Zhang}\affiliation{Shandong University, Qingdao, Shandong 266237}
\author{Y.~Zhang}\affiliation{Guangxi Normal University, Guilin, 541004}
\author{Z.~Zhang}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Z.~Zhang}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{F.~Zhao}\affiliation{Lanzhou University}
\author{J.~Zhao}\affiliation{Fudan University, Shanghai, 200433 }
\author{M.~Zhao}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~Zhou}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{Y.~Zhou}\affiliation{Central China Normal University, Wuhan, Hubei 430079 }
\author{X.~Zhu}\affiliation{Tsinghua University, Beijing 100084}
\author{M.~Zurek}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{M.~Zyzak}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}

\collaboration{STAR Collaboration}\noaffiliation

==> authorlistb_IOP.tex <==
\author{
B.~E.~Aboona$^{57}$,
J.~Adam$^{17}$,
L.~Adamczyk$^{3}$,
I.~Aggarwal$^{44}$,
M.~M.~Aggarwal$^{44}$,
Z.~Ahammed$^{64}$,
E.~C.~Aschenauer$^{7}$,
S.~Aslam$^{29}$,
J.~Atchison$^{2}$,
V.~Bairathi$^{55}$,
X.~Bao$^{51}$,
K.~Barish$^{12}$,
S.~Behera$^{28}$,
R.~Bellwied$^{25}$,
P.~Bhagat$^{32}$,
A.~Bhasin$^{32}$,
S.~Bhatta$^{54}$,
S.~R.~Bhosale$^{3}$,
J.~Bielcik$^{17}$,
J.~Bielcikova$^{42}$,
J.~D.~Brandenburg$^{43}$,
C.~Broodo$^{25}$,
X.~Z.~Cai$^{52}$,
H.~Caines$^{68}$,
M.~Calder{\'o}n~de~la~Barca~S{\'a}nchez$^{10}$,
D.~Cebra$^{10}$,
J.~Ceska$^{17}$,
I.~Chakaberia$^{36}$,
P.~Chaloupka$^{17}$,
B.~K.~Chan$^{11}$,
Z.~Chang$^{30}$,
A.~Chatterjee$^{19}$,
D.~Chen$^{12}$,
J.~Chen$^{51}$,
J.~H.~Chen$^{22}$,
Q.~Chen$^{23}$,
Z.~Chen$^{51}$,
J.~Cheng$^{59}$,
Y.~Cheng$^{11}$,
W.~Christie$^{7}$,
X.~Chu$^{7}$,
S.~Corey$^{43}$,
H.~J.~Crawford$^{9}$,
M.~Csan\'{a}d$^{20}$,
G.~Dale-Gau$^{14}$,
A.~Das$^{17}$,
I.~M.~Deppner$^{24}$,
A.~Deshpande$^{54}$,
A.~Dhamija$^{44}$,
A.~Dimri$^{54}$,
P.~Dixit$^{27}$,
X.~Dong$^{36}$,
J.~L.~Drachenberg$^{2}$,
E.~Duckworth$^{33}$,
J.~C.~Dunlop$^{7}$,
J.~Engelage$^{9}$,
G.~Eppley$^{46}$,
S.~Esumi$^{60}$,
O.~Evdokimov$^{14}$,
O.~Eyser$^{7}$,
R.~Fatemi$^{34}$,
S.~Fazio$^{8}$,
Y.~Feng$^{45}$,
E.~Finch$^{53}$,
Y.~Fisyak$^{7}$,
F.~A.~Flor$^{68}$,
C.~Fu$^{31}$,
T.~Fu$^{51}$,
C.~A.~Gagliardi$^{57}$,
T.~Galatyuk$^{18}$,
T.~Gao$^{51}$,
F.~Geurts$^{46}$,
N.~Ghimire$^{56}$,
A.~Gibson$^{63}$,
K.~Gopal$^{28}$,
X.~Gou$^{51}$,
D.~Grosnick$^{63}$,
A.~Gu$^{26}$,
A.~Gupta$^{32}$,
A.~Hamed$^{5}$,
X.~Han$^{43}$,
S.~Harabasz$^{18}$,
M.~D.~Harasty$^{10}$,
J.~W.~Harris$^{68}$,
H.~Harrison-Smith$^{34}$,
L.~B.~ Havener$^{68}$,
X.~H.~He$^{31}$,
Y.~He$^{51}$,
N.~Herrmann$^{24}$,
L.~Holub$^{17}$,
C.~Hu$^{61}$,
Q.~Hu$^{31}$,
Y.~Hu$^{36}$,
H.~Huang$^{41}$,
H.~Z.~Huang$^{11}$,
S.~L.~Huang$^{54}$,
T.~Huang$^{14}$,
Y.~Huang$^{59}$,
Y.~Huang$^{13}$,
T.~J.~Humanic$^{43}$,
M.~Isshiki$^{60}$,
W.~W.~Jacobs$^{30}$,
A.~Jalotra$^{32}$,
C.~Jena$^{28}$,
A.~Jentsch$^{7}$,
Y.~Ji$^{36}$,
J.~Jia$^{54,7}$,
C.~Jin$^{46}$,
N.~ Jindal$^{43}$,
X.~Ju$^{48}$,
E.~G.~Judd$^{9}$,
S.~Kabana$^{55}$,
D.~Kalinkin$^{34}$,
K.~Kang$^{59}$,
D.~Kapukchyan$^{12}$,
K.~Kauder$^{7}$,
D.~Keane$^{33}$,
A.~ Khanal$^{66}$,
Y.~V.~Khyzhniak$^{43}$,
D.~P.~Kiko\l{}a~$^{65}$,
J.~Kim$^{7}$,
D.~Kincses$^{20}$,
I.~Kisel$^{21}$,
A.~Kiselev$^{7}$,
A.~G.~Knospe$^{37}$,
H.~S.~Ko$^{36}$,
J.~Ko{\l}a\'s$^{65}$,
B.~Korodi$^{43}$,
L.~K.~Kosarzewski$^{43}$,
L.~Kumar$^{44}$,
M.~C.~Labonte$^{10}$,
R.~Lacey$^{54}$,
J.~M.~Landgraf$^{7}$,
C.~ Larson$^{34}$,
J.~Lauret$^{7}$,
A.~Lebedev$^{7}$,
J.~H.~Lee$^{7}$,
Y.~H.~Leung$^{24}$,
C.~Li$^{13}$,
D.~Li$^{48}$,
H-S.~Li$^{45}$,
H.~Li$^{67}$,
H.~Li$^{23}$,
W.~Li$^{46}$,
X.~Li$^{48}$,
X.~Li$^{48}$,
Y.~Li$^{59}$,
Z.~Li$^{49}$,
Z.~Li$^{48}$,
X.~Liang$^{12}$,
Y.~Liang$^{33}$,
R.~Licenik$^{42,17}$,
T.~Lin$^{51}$,
Y.~Lin$^{23}$,
M.~A.~Lisa$^{43}$,
C.~Liu$^{31}$,
G.~Liu$^{49}$,
H.~Liu$^{13}$,
L.~Liu$^{13}$,
Z.~Liu$^{13}$,
T.~Ljubicic$^{46}$,
O.~Lomicky$^{17}$,
R.~S.~Longacre$^{7}$,
E.~M.~Loyd$^{12}$,
T.~Lu$^{31}$,
J.~Luo$^{48}$,
X.~F.~Luo$^{13}$,
L.~Ma$^{22}$,
R.~Ma$^{7}$,
Y.~G.~Ma$^{22}$,
D.~Mallick$^{65}$,
R.~Manikandhan$^{25}$,
S.~Margetis$^{33}$,
C.~Markert$^{58}$,
O.~Matonoha$^{17}$,
O.~Mezhanska$^{17}$,
K.~Mi$^{13}$,
S.~Mioduszewski$^{57}$,
B.~Mohanty$^{40}$,
B.~Mondal$^{40}$,
M.~M.~Mondal$^{40}$,
I.~Mooney$^{68}$,
J.~Mrazkova$^{42,17}$,
M.~I.~Nagy$^{20}$,
C.~J.~Naim$^{54}$,
A.~S.~Nain$^{44}$,
J.~D.~Nam$^{56}$,
M.~Nasim$^{27}$,
H.~Nasrulloh$^{48}$,
D.~Neff$^{11}$,
J.~M.~Nelson$^{9}$,
M.~Nie$^{51}$,
G.~Nigmatkulov$^{14}$,
T.~Niida$^{60}$,
T.~Nonaka$^{60}$,
G.~Odyniec$^{36}$,
A.~Ogawa$^{7}$,
S.~Oh$^{50}$,
K.~Okubo$^{60}$,
B.~S.~Page$^{7}$,
S.~Pal$^{17}$,
A.~Pandav$^{36}$,
A.~Panday$^{27}$,
A.~K.~Pandey$^{31}$,
T.~Pani$^{47}$,
A.~Paul$^{12}$,
S.~Paul$^{54}$,
D.~Pawlowska$^{65}$,
C.~Perkins$^{9}$,
J.~Pluta$^{65}$,
B.~R.~Pokhrel$^{56}$,
I.~D.~ Ponce~Pinto$^{68}$,
M.~Posik$^{56}$,
S.~Prodhan$^{28}$,
T.~L.~Protzman$^{37}$,
A.~Prozorov$^{17}$,
V.~Prozorova$^{17}$,
N.~K.~Pruthi$^{44}$,
M.~Przybycien$^{3}$,
J.~Putschke$^{66}$,
Z.~Qin$^{59}$,
H.~Qiu$^{31}$,
S.~K.~Radhakrishnan$^{33}$,
A.~Rana$^{44}$,
R.~L.~Ray$^{58}$,
R.~Reed$^{37}$,
C.~W.~ Robertson$^{45}$,
M.~Robotkova$^{42,17}$,
M.~ A.~Rosales~Aguilar$^{34}$,
D.~Roy$^{47}$,
P.~Roy~Chowdhury$^{65}$,
L.~Ruan$^{7}$,
A.~K.~Sahoo$^{27}$,
N.~R.~Sahoo$^{28}$,
H.~Sako$^{60}$,
S.~Salur$^{47}$,
S.~S.~Sambyal$^{32}$,
J.~K.~Sandhu$^{37}$,
S.~Sato$^{60}$,
B.~C.~Schaefer$^{37}$,
N.~Schmitz$^{38}$,
F-J.~Seck$^{18}$,
J.~Seger$^{16}$,
R.~Seto$^{12}$,
P.~Seyboth$^{38}$,
N.~Shah$^{29}$,
P.~V.~Shanmuganathan$^{7}$,
T.~Shao$^{22}$,
M.~Sharma$^{32}$,
N.~Sharma$^{27}$,
R.~Sharma$^{28}$,
S.~R.~ Sharma$^{28}$,
A.~I.~Sheikh$^{33}$,
D.~Shen$^{51}$,
D.~Y.~Shen$^{31}$,
K.~Shen$^{48}$,
S.~Shi$^{13}$,
Y.~Shi$^{51}$,
F.~Si$^{48}$,
J.~Singh$^{55}$,
S.~Singha$^{31}$,
P.~Sinha$^{28}$,
M.~J.~Skoby$^{6,45}$,
N.~Smirnov$^{68}$,
Y.~S\"{o}hngen$^{24}$,
Y.~Song$^{68}$,
T.~D.~S.~Stanislaus$^{63}$,
M.~Stefaniak$^{43}$,
Y.~Su$^{48}$,
M.~Sumbera$^{42}$,
X.~Sun$^{31}$,
Y.~Sun$^{48}$,
B.~Surrow$^{56}$,
M.~Svoboda$^{42,17}$,
Z.~W.~Sweger$^{10}$,
A.~C.~Tamis$^{68}$,
A.~H.~Tang$^{7}$,
Z.~Tang$^{48}$,
T.~Tarnowsky$^{39}$,
J.~H.~Thomas$^{36}$,
A.~R.~Timmins$^{25}$,
D.~Tlusty$^{16}$,
T.~Todoroki$^{60}$,
D.~Torres~Valladares$^{46}$,
S.~Trentalange$^{11}$,
P.~Tribedy$^{7}$,
S.~K.~Tripathy$^{65}$,
T.~Truhlar$^{17}$,
B.~A.~Trzeciak$^{17}$,
O.~D.~Tsai$^{11,7}$,
C.~Y.~Tsang$^{33,7}$,
Z.~Tu$^{7}$,
J.~Tyler$^{57}$,
T.~Ullrich$^{7}$,
D.~G.~Underwood$^{4,63}$,
G.~Van~Buren$^{7}$,
J.~Vanek$^{7}$,
I.~Vassiliev$^{21}$,
F.~Videb{\ae}k$^{7}$,
S.~A.~Voloshin$^{66}$,
F.~Wang$^{45}$,
G.~Wang$^{11}$,
J.~S.~Wang$^{26}$,
J.~Wang$^{51}$,
K.~Wang$^{48}$,
X.~Wang$^{51}$,
Y.~Wang$^{48}$,
Y.~Wang$^{13}$,
Y.~Wang$^{59}$,
Z.~Wang$^{51}$,
A.~J.~Watroba$^{3}$,
J.~C.~Webb$^{7}$,
P.~C.~Weidenkaff$^{24}$,
G.~D.~Westfall$^{39}$,
D.~Wielanek$^{65}$,
H.~Wieman$^{36}$,
G.~Wilks$^{14}$,
S.~W.~Wissink$^{30}$,
R.~Witt$^{62}$,
C.~P.~Wong$^{7}$,
J.~Wu$^{13}$,
J.~Wu$^{61}$,
X.~Wu$^{11}$,
X,Wu$^{48}$,
B.~Xi$^{22}$,
Z.~G.~Xiao$^{59}$,
G.~Xie$^{61}$,
W.~Xie$^{45}$,
H.~Xu$^{26}$,
N.~Xu$^{36}$,
Q.~H.~Xu$^{51}$,
Y.~Xu$^{51}$,
Y.~Xu$^{13}$,
Z.~Xu$^{33}$,
Z.~Xu$^{11}$,
G.~Yan$^{51}$,
Z.~Yan$^{54}$,
C.~Yang$^{51}$,
Q.~Yang$^{51}$,
S.~Yang$^{49}$,
Y.~Yang$^{1,41}$,
Z.~Ye$^{49}$,
Z.~Ye$^{36}$,
L.~Yi$^{51}$,
Y.~Yu$^{51}$,
H.~Zbroszczyk$^{65}$,
W.~Zha$^{48}$,
C.~Zhang$^{22}$,
D.~Zhang$^{49}$,
J.~Zhang$^{51}$,
S.~Zhang$^{15}$,
W.~Zhang$^{49}$,
X.~Zhang$^{31}$,
Y.~Zhang$^{31}$,
Y.~Zhang$^{48}$,
Y.~Zhang$^{51}$,
Y.~Zhang$^{23}$,
Z.~Zhang$^{7}$,
Z.~Zhang$^{14}$,
F.~Zhao$^{35}$,
J.~Zhao$^{22}$,
M.~Zhao$^{7}$,
S.~Zhou$^{13}$,
Y.~Zhou$^{13}$,
X.~Zhu$^{59}$,
M.~Zurek$^{4,7}$,
M.~Zyzak$^{21}$
}

%\\[1ex]


\address{\rm{(STAR Collaboration)}}

%\\[1ex]

\address{$^{1}$Academia Sinica}
\address{$^{2}$Abilene Christian University, Abilene, Texas   79699}
\address{$^{3}$AGH University of Krakow, FPACS, Cracow 30-059, Poland}
\address{$^{4}$Argonne National Laboratory, Argonne, Illinois 60439}
\address{$^{5}$American University in Cairo, New Cairo 11835, Egypt}
\address{$^{6}$Ball State University, Muncie, Indiana, 47306}
\address{$^{7}$Brookhaven National Laboratory, Upton, New York 11973}
\address{$^{8}$University of Calabria \& INFN-Cosenza, Rende 87036, Italy}
\address{$^{9}$University of California, Berkeley, California 94720}
\address{$^{10}$University of California, Davis, California 95616}
\address{$^{11}$University of California, Los Angeles, California 90095}
\address{$^{12}$University of California, Riverside, California 92521}
\address{$^{13}$Central China Normal University, Wuhan, Hubei 430079 }
\address{$^{14}$University of Illinois at Chicago, Chicago, Illinois 60607}
\address{$^{15}$Chongqing University, Chongqing, 401331}
\address{$^{16}$Creighton University, Omaha, Nebraska 68178}
\address{$^{17}$Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\address{$^{18}$Technische Universit\"at Darmstadt, Darmstadt 64289, Germany}
\address{$^{19}$National Institute of Technology Durgapur, Durgapur - 713209, India}
\address{$^{20}$ELTE E\"otv\"os Lor\'and University, Budapest, Hungary H-1117}
\address{$^{21}$Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\address{$^{22}$Fudan University, Shanghai, 200433 }
\address{$^{23}$Guangxi Normal University, Guilin, 541004}
\address{$^{24}$University of Heidelberg, Heidelberg 69120, Germany }
\address{$^{25}$University of Houston, Houston, Texas 77204}
\address{$^{26}$Huzhou University, Huzhou, Zhejiang  313000}
\address{$^{27}$Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\address{$^{28}$Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\address{$^{29}$Indian Institute Technology, Patna, Bihar 801106, India}
\address{$^{30}$Indiana University, Bloomington, Indiana 47408}
\address{$^{31}$Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\address{$^{32}$University of Jammu, Jammu 180001, India}
\address{$^{33}$Kent State University, Kent, Ohio 44242}
\address{$^{34}$University of Kentucky, Lexington, Kentucky 40506-0055}
\address{$^{35}$Lanzhou University}
\address{$^{36}$Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\address{$^{37}$Lehigh University, Bethlehem, Pennsylvania 18015}
\address{$^{38}$Max-Planck-Institut f\"ur Physik, Munich 80805, Germany}
\address{$^{39}$Michigan State University, East Lansing, Michigan 48824}
\address{$^{40}$National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\address{$^{41}$National Cheng Kung University, Tainan 70101 }
\address{$^{42}$Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}
\address{$^{43}$The Ohio State University, Columbus, Ohio 43210}
\address{$^{44}$Panjab University, Chandigarh 160014, India}
\address{$^{45}$Purdue University, West Lafayette, Indiana 47907}
\address{$^{46}$Rice University, Houston, Texas 77251}
\address{$^{47}$Rutgers University, Piscataway, New Jersey 08854}
\address{$^{48}$University of Science and Technology of China, Hefei, Anhui 230026}
\address{$^{49}$South China Normal University, Guangzhou, Guangdong 510631}
\address{$^{50}$Sejong University, Seoul, 05006, South Korea}
\address{$^{51}$Shandong University, Qingdao, Shandong 266237}
\address{$^{52}$Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\address{$^{53}$Southern Connecticut State University, New Haven, Connecticut 06515}
\address{$^{54}$State University of New York, Stony Brook, New York 11794}
\address{$^{55}$Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Arica 1000000, Chile}
\address{$^{56}$Temple University, Philadelphia, Pennsylvania 19122}
\address{$^{57}$Texas A\&M University, College Station, Texas 77843}
\address{$^{58}$University of Texas, Austin, Texas 78712}
\address{$^{59}$Tsinghua University, Beijing 100084}
\address{$^{60}$University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\address{$^{61}$University of Chinese Academy of Sciences, Beijing, 101408}
\address{$^{62}$United States Naval Academy, Annapolis, Maryland 21402}
\address{$^{63}$Valparaiso University, Valparaiso, Indiana 46383}
\address{$^{64}$Variable Energy Cyclotron Centre, Kolkata 700064, India}
\address{$^{65}$Warsaw University of Technology, Warsaw 00-661, Poland}
\address{$^{66}$Wayne State University, Detroit, Michigan 48201}
\address{$^{67}$Wuhan University of Science and Technology, Wuhan, Hubei 430065}
\address{$^{68}$Yale University, New Haven, Connecticut 06520}
%\address{{$^{*}${\rm Deceased}}}

==> authornolist.tex <==
\address{\rm{(STAR Collaboration)}}

==> comment.tex <==
% 目前文章中还需完善，目前先放置后续一起处理的一些问题：

% 文章的书写 摘要，图在文章中的描述都是本人参考七八篇STAR LHC最近发的prl写的，都是偏技术细节偏提供数字，图的表述都很直白Figure 1 shows ...这种，可以说PRL的风格就是这样，技术细节喜欢定量的刊刊

%____________________________________________________________
% DS 在mass上的A2 enhangement的显著度，需要跑一整遍程序之后更新，包括具体的DS和rho的A2 在0.6-0.9 mass 积分区间的值 （目前未填或用nsigma表示）
%____________________________________________________________

%图暂时用png，因为prl prefers eps格式，适合编译但无法直接看，现在只看内容，都改完后把图也调整后存eps

% (TODO) 可能要在introduction里提一嘴HERA那个B/A的测量

% 图里 EPA-VMD Soding 我改成 Non-resonance production model 了就是NRP，自己起的名，不合适的话我们讨论起个名

% 有很多细节比如NRP怎么算的（文章未发表）是不清楚无法重复可能会被一直问的，PRL 有个 END Matter专门写这种，不知道我们要不要写个end matter，大部分prl没写，也有少部分写了

% reference的格式后期再调整，大部分人的prl好像reference不加标题



==> instituional_diff_test_EESI.tex <==
%\label{sec:dataselection}

% physics：
% 1. mass ordering image the nucleus
% %%%% nuclear force (need pi N cross section)
% 2. novel probe for deep understanding the interference
% 3. comparason to rho:    
% how does different photon hadronic structure
% production mechanics
% affect imagining the nucleus and the interference


% Introduction:
% nuclear and vacuum structure
% photoproduction used for parton dis both sides
% Entanglement interference
% unsolved issue & It is of great interest to investigate...
% In this Letter, we present
% The data and the trigger
% Event track pid cut and observable recon
% 

%The vacuum under the extremely strong electromagnetic field produced in relativistic heavy ion collisions has a subtle partonic structure. The photon induced processes, vector meson photoproduction and photon photon process, have been extensively measured

%The extremely strong electromagnetic field generated in the relativistic heavy-ion collisions can be described as a co-moving photon cloud with beams~\cite{weizsacker1934ausstrahlung,williams1934nature}, and thus enables photon nuclear interactions~\cite{krauss1997photon}. In the scenario of such interactions, a photon fluctuates into a virtual vector meson or hadron-antihadron pair, which then scatters off the nucleus by Pomeron exchange (finite sum of gluon ladders). Therefore, photon-nuclear interactions provide a unique probe of the photon's hadronic structure~\cite{bauer1978hadronic,AbdulKhalek:2021gbh,Li:2022kwn} and serve as a complementary tool for studying key nuclear properties, including the nuclear gluon distributions~\cite{guzey2013exclusive} and the overall nuclear size~\cite{sciadv.abq3903,Klein:1999qj}.
Ultra-strong electromagnetic fields in relativistic heavy-ion collisions \DIFdelbegin \DIFdel{manifest }\DIFdelend \DIFaddbegin \DIFadd{are manifested }\DIFaddend as a comoving photon cloud accompanying the nuclei~\cite{weizsacker1934ausstrahlung,williams1934nature}, enabling photonuclear interactions. In these processes, a photon fluctuates into a virtual vector meson or hadron-antihadron pair, which scatters via Pomeron exchange (gluonic exchanges). Such interactions provide a unique probe of the photon's hadronic structure~\cite{bauer1978hadronic,AbdulKhalek:2021gbh,Li:2022kwn} and serve as a complementary tool for studying key nuclear properties, including nuclear gluon distributions~\cite{guzey2013exclusive} and the overall \DIFdelbegin \DIFdel{nuclear size }\DIFdelend \DIFaddbegin \DIFadd{size of the nucleus}\DIFaddend ~\cite{sciadv.abq3903,Klein:1999qj}.
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend %For a quasi-real photon with spin-1, dissociation processes must adhere to angular momentum conservation. The photon may fluctuate into either (\romannumeral1) a virtual vector meson, which retains the photon’s spin and parity quantum numbers $(J^{PC}=1^{--})$, or (\romannumeral2) a virtual hadron-antihadron pair, giving rise to non-resonant photoproduction, known as the Drell-S${\rm \ddot{o}ding}$ process. 
\DIFaddbegin 

\DIFaddend A quasi-real spin-1 photon can fluctuate into (\romannumeral1) a virtual vector meson $(J^{PC}=1^{--})$, or (\romannumeral2) a virtual hadron-antihadron pair, giving rise to non-resonant photoproduction, known as the Drell-S${\rm \ddot{o}ding}$ process. 
In the case of scalar mesons such as $\pi^{+}\pi^{-}$, the angular momentum is encoded in the pair orbital momentum, resulting in quantum entanglement between the $\pi^{+}$ and $\pi^{-}$ \DIFaddbegin \DIFadd{in the relative-motion spatial wave function}\DIFaddend . A separate quantum phenomenon arises from the collision geometry: since both nuclei can act as photon emitters or targets, the emission source (nucleus A or B) becomes \DIFdelbegin \DIFdel{almost }\DIFdelend indistinguishable, establishing a ``double-slit'' interference pattern at the femtometer scale~\cite{sciadv.abq3903,PhysRevD.103.033007}. This interference induces second-order cosine oscillations in the asymmetries of the decay angular $\Delta\phi$ distributions~\cite{xing2020cos}. \DIFdelbegin \DIFdel{In the Drell-S${\rm \ddot{o}ding}$ mechanism, the relativistic $\pi^{+}\pi^{-}$ pair emerges via photon-nuclear interaction and rapidly separates in nearly opposite directions. %DIF < at relativistic speeds. 
The pair resembles an Einstein-Podolsky-Rosen (EPR) system~\mbox{%DIFAUXCMD
\cite{Brandenburg:2024ksp} }\hspace{0pt}%DIFAUXCMD
with no further information transmission after production. 
It is of great interest to investigate in depth the interference and entanglement in }\DIFdelend %DIF > In the Drell-S${\rm \ddot{o}ding}$ mechanism, the relativistic $\pi^{+}\pi^{-}$ pair emerges via a photon-nuclear interaction and rapidly separates in nearly opposite directions. %at relativistic speeds.
\DIFaddbegin \DIFadd{In this picture, interference at the pair level arises from the indistinguishability of }\DIFaddend the \DIFdelbegin \DIFdel{Drell-S${\rm \ddot{o}ding}$ process.
}%DIFDELCMD < 

%DIFDELCMD < %%%
%DIF < It is a chance to explore the effect of decay in comparison to the production with an intermediate state such as $\rho^0$. 
\DIFdelend \DIFaddbegin \DIFadd{photon emission sources, while the entanglement of the $\pi^{+}\pi^{-}$ final state allows this interference to manifest in the measured decay angular distributions, giving rise to EESI effect.
%DIF > As with all Einstein-Podolsky-Rosen (EPR) systems, it is of great interest to investigate in depth the interference and entanglement in the Drell-S${\rm \ddot{o}ding}$ process.
}\DIFaddend 

The \DIFdelbegin \DIFdel{Drell-S}\DIFdelend \DIFaddbegin \DIFadd{Drell–S}\DIFaddend ${\rm \ddot{o}ding}$ process \DIFaddbegin \DIFadd{is a sensitive probe of the nuclear gluon structure, nuclear gluon saturation, and shadowing effects~\mbox{%DIFAUXCMD
\cite{ZEUS:1997rof,Laget:2019tou}}\hspace{0pt}%DIFAUXCMD
.
It }\DIFaddend has two dominant diagrams\DIFdelbegin \DIFdel{through virtual $\pi^+/\pi^-$-nucleus scattering}\DIFdelend \DIFaddbegin \DIFadd{, corresponding to $\pi^+-$nucleus and $\pi^--$nucleus scattering~\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,bolz2015photoproduction}}\hspace{0pt}%DIFAUXCMD
, as }\DIFaddend depicted in Fig.~\ref{fig:1}. \DIFdelbegin \DIFdel{And another for the gauge invariance~\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,bolz2015photoproduction}}\hspace{0pt}%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{A sub-leading $\pi^+\pi^--$nucleus coupling diagram is included to ensure gauge invariance\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend .
In 1960, Drell first proposed \DIFdelbegin \DIFdel{the diagrams of this process as promising contributions }\DIFdelend \DIFaddbegin \DIFadd{these diagrams as promising contributors }\DIFaddend to secondary beams \DIFdelbegin \DIFdel{via the $\gamma \rightarrow \pi^+\pi^-$ process }\DIFdelend at SLAC~\cite{drell1960production}. Later in 1966, S${\rm \ddot{o}ding}$ \DIFdelbegin \DIFdel{calculated them }\DIFdelend \DIFaddbegin \DIFadd{carried out a full calculation of the $\gamma p \to \pi^+\pi^- p$ process and used it }\DIFaddend to explain the observed skewing of the $\rho^0$ resonance peak~\cite{soding1966apparent}. 
\DIFdelbegin \DIFdel{Compared to the resonance $\rho^0$, the direct $\pi^+\pi^-$ is more loosely bounded with a larger dipole size, corresponding to a smaller pair $p_T$ even at the same photon energy. With such a system scattering from the nucleus via a Pomeron, }\DIFdelend %DIF > In diffractive photoproduction, the momentum-transfer t distribution is known to reflect the transverse spatial structure of the interaction. In particular, a steeper t dependence is generally associated with larger effective transverse configurations~\cite{Kuroda:2017ogq,Kowalski:2006hc,Nemchik:1996cw}. In this context, comparing the t spectra of the resonant and non-resonant $\pi^+\pi^-$ contributions provides a way to probe potential differences in their underlying transverse dipole size.
\DIFaddbegin \DIFadd{In diffractive photoproduction, the momentum-transfer t distribution primarily reflects the transverse spatial profile of the target through its form factor. At the same time, it can also be sensitive to }\DIFaddend the \DIFdelbegin \DIFdel{Drell-S${\rm \ddot{o}ding}$ process serves as a sensitive probe of the nuclear gluon structure, the nuclear saturation and shadowing effect in $\pi^+/\pi^-$-p diffraction scattering~\mbox{%DIFAUXCMD
\cite{ZEUS:1997rof,Laget:2019tou}}\hspace{0pt}%DIFAUXCMD
.
%DIF < In addition, the 
}%DIFDELCMD < 

%DIFDELCMD < %%%
%DIF < Recently, as  it was realized that the Drell-S${\rm \ddot{o}ding}$ process
%DIF < Hereinafter, the Drell-S${\rm \ddot{o}ding}$ process was introduced to modify the $\rho^0$ mass shape in phenomenological models and measurements.%in most of measurements of the exclusive $\pi^+\pi^-$ production in
%DIF < Due to the specific one-pion-exchange mechanism and the smallness of the $\pi$ mass, the Drell-S${\rm \ddot{o}ding}$ process is expected to be softer than $\rho^0$ photoproduction and can be correlated to hadron-induced processes~\cite{pumplin1970diffraction}.
\DIFdelend \DIFaddbegin \DIFadd{transverse size of the interacting dipole via the convolution of the photon and hadronic wavefunctions with the scattering amplitude. In particular, a steeper t dependence is generally associated with larger effective transverse configurations~\mbox{%DIFAUXCMD
\cite{Kuroda:2017ogq,Kowalski:2006hc,Nemchik:1996cw}}\hspace{0pt}%DIFAUXCMD
.
In this context, comparing the t spectra of the resonant and non-resonant $\pi^+\pi^-$ contributions within the same mass and rapidity range provides a way to probe potential differences in their underlying transverse dipole sizes.
%DIF > Compared to the resonance $\rho^0$, the direct $\pi^+\pi^-$ is more loosely bound with a larger dipole size and corresponding to a smaller pair $p_T$, as implied by the transverse size–momentum uncertainty relation.
%DIF > It is dominated by the virtual $\pi$–nucleus scattering diagrams~\cite{pumplin1970diffraction,bolz2015photoproduction}, for both $\pi^+/$–nucleus and $\pi^-$–nucleus scattering as depicted in Fig.~\ref{fig:1}.
}\DIFaddend 

Vector meson photoproduction, e.g., $\rho^0$ and $J/\psi$, has been measured extensively in ultraperipheral collisions (UPCs) of heavy ions~\cite{alice2021coherent,acharya2019coherent,STAR:2017enh,abelev2008rho,STAR:2019yox,STAR:2002caw,afanasiev2009photoproduction,guzey2013evidence,ALICE:2020ugp,ALICE:2024ife,collaboration2021first,GlueX:2024erj,Pybus:2024ifi,GlueX:2019mkq}. 
However, the non-resonant \DIFdelbegin \DIFdel{Drell-Söding }\DIFdelend \DIFaddbegin \DIFadd{Drell-S${\rm \ddot{o}ding}$ }\DIFaddend process remains poorly characterized due to its small cross section and overlap with resonant $\rho^0$.
%DIF > The Drell-S${\rm \ddot{o}ding}$ term cannot be isolated event-by-event and is extracted through its interference with the $\rho^0$ photoproduction.
\DIFaddbegin \DIFadd{The Drell-S${\rm \ddot{o}ding}$ term cannot be isolated on an event-by-event basis and is extracted statistically after subtracting known contributions, relying on its interference with the $\rho^0$ photoproduction.
}\DIFaddend In previous $\rho^0$ measurements, the Drell-S${\rm \ddot{o}ding}$ component is treated with an unknown amplitude formulated as a constant~\cite{STAR:2017enh,abelev2008rho,STAR:2019yox,STAR:2002caw,ALICE:2020ugp} or a parameterised function~\cite{H1:2020lzc,ZEUS:2011tzw}. 
\DIFdelbegin \DIFdel{However, when isolating the }\DIFdelend %DIF > However, when isolating the Drell-S${\rm \ddot{o}ding}$ contribution, replacing the constant approximation with a model-calculated spectrum results in a deviation over $15\%$ of the extracted Drell-S${\rm \ddot{o}ding}$ cross section. 
\DIFaddbegin \DIFadd{The extracted }\DIFaddend Drell-S${\rm \ddot{o}ding}$ contribution \DIFdelbegin \DIFdel{, replacing the constant approximation with a model-calculated spectrum results in a deviation over $15\%$ of the extracted Drell-S${\rm \ddot{o}ding}$ cross section}\DIFdelend \DIFaddbegin \DIFadd{depends on the assumed mass dependence of this term}\DIFaddend . Therefore, adopting a more realistic spectrum derived from model calculations \DIFdelbegin \DIFdel{is crucial to achieve }\DIFdelend \DIFaddbegin \DIFadd{would be desirable to achieve a more }\DIFaddend precise measurements of the Drell-S${\rm \ddot{o}ding}$ process.
%DIF > Experimentally, the Drell-S${\rm \ddot{o}ding}$ contribution cannot be isolated event-by-event; instead, it is extracted through its interference with the $\rho^0$ amplitude that shapes the exclusive $\pi^+\pi^-$ mass spectrum.
With growing interest in exclusive hadronic pair production~\cite{sciadv.abq3903,Brandenburg:2024ksp,TOTEM:2024aso,ALICE:2023kgv,STAR:2020dzd,ATLAS:2022uef}, precise measurements of the Drell-S${\rm \ddot{o}ding}$ process offer a new handle to quantify decay-induced effects in nuclear tomography and \DIFdelbegin \DIFdel{entanglement enabled spin-interference (EESI ) }\DIFdelend \DIFaddbegin \DIFadd{EESI }\DIFaddend via comparisons with $\rho^0$ photoproduction. A precise characterization of the Drell-S${\rm \ddot{o}ding}$ process is also \DIFdelbegin \DIFdel{essential }\DIFdelend \DIFaddbegin \DIFadd{important }\DIFaddend for disentangling excited $\rho^0$ states, e.g., $\rho(1450)$ and $\rho(1700)$, in exclusive $\pi^+\pi^-$ production~\cite{ALICE:2020ugp}.
%The Drell-S${\rm \ddot{o}ding}$ process could provide a novel probe to the nuclear gluon densities
%provides a unique opportunity to study the photon hadronic $\pi^+\pi^-$ and $\rho^0$ structure by comparison to $\rho^0$ photoproduction and the gluonic structure of nucleus.
%The variation for the Drell-S${\rm \ddot{o}ding}$ mass shape implemented has a negligible impact on the obtained $\rho^0$ cross section but leads to an obvious uncertainty ($\sim15\%$) for the Drell-S${\rm \ddot{o}ding}$. It is one of the most pressing tasks to apply a more real form for precise measurement of the Drell-S${\rm \ddot{o}ding}$ process in high energy nuclear UPC physics.

% main content of the measurement
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend In this Letter, we report a comprehensive analysis for a series of simultaneous measurements of exclusive $\pi^{+}\pi^{-}$ production. For the first time, (\romannumeral1) the $|t|$ dependence of the Drell-S${\rm \ddot{o}ding}$ process cross section is precisely measured; (\romannumeral2) EESI for the Drell-S${\rm \ddot{o}ding}$ process is measured through ${\rm A_{2\Delta\phi}}$; \DIFaddbegin \DIFadd{and }\DIFaddend (\romannumeral3) \DIFdelbegin \DIFdel{We measure how }\DIFdelend \DIFaddbegin \DIFadd{the dependence of }\DIFaddend ${\rm A_{2\Delta\phi}}$ \DIFaddbegin \DIFadd{on the pair invariant mass is measured }\DIFaddend for exclusive $\pi^+\pi^-$ pair production\DIFdelbegin \DIFdel{depends on pair invariant mass related to the incident photon energy. The }\DIFdelend \DIFaddbegin \DIFadd{. Finally, the }\DIFaddend ${\rm A_{2\Delta\phi}}$ data are compared with vector meson dominant (VMD)~\cite{PhysRevD.103.033007,Zha:2018jin} and non-resonance production (NRP) calculations~\DIFdelbegin \DIFdel{\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,Zha:2018jin}}\hspace{0pt}%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,Zha:2018jin,Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend .

\DIFdelbegin %DIFDELCMD < \begin{figure}[h]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.45\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{Figure1 pancake nucleus.png}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{Schematic view of the production mechanism for Drell-S${\rm \ddot{o}ding}$ process. A virtual photon fluctuates into an entangled $\pi^{+}\pi^{-}$ pair during the strong interaction time ($\sim 2\times10^{-24}$s). One single virtual $\pi^{+}/\pi^{-}$ is diffraction-scattered on the nucleus. The wavy structures represent local energy fluctuations in the strong electromagnetic field, while the associated blue and red balls depict short-lived pair fluctuations due to the local energy excitations. }
%DIFDELCMD <   \label{fig:1}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\DIFdelend %DIF >  \begin{figure}[h]
%DIF >    \centering
%DIF >    \begin{minipage}{0.45\textwidth}
%DIF >      \includegraphics[width=\textwidth]{Figure1 pancake nucleus.png}
%DIF >    \end{minipage}
%DIF >    \caption{A schematic diagram showing the production of entangled pions via the Drell-S${\rm \ddot{o}ding}$ process. A virtual photon fluctuates into an entangled $\pi^{+}\pi^{-}$ pair during the strong interaction time and one of the pions is diffraction-scattered off the nucleus. The wavy structures in the background represent local energy fluctuations in the strong electromagnetic field, while the associated blue and red balls depict short-lived pair fluctuations due to the local energy excitations. }
%DIF >    \label{fig:1}
%DIF >  \end{figure}
\DIFaddbegin \begin{figure}[t]
\centering

\begin{minipage}{0.325\columnwidth}
\centering
\includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_1_largetext.eps}\hfill
%\\ (\romannumeral1)
\end{minipage}
\begin{minipage}{0.325\columnwidth}
\centering
\includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_2_largetext.eps}\hfill
%\\ (\romannumeral2)
\end{minipage}
%\vspace{0.2cm}
\begin{minipage}{0.325\columnwidth}
\centering
\includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_3_largetext.eps}
% \\ (\romannumeral3)
\end{minipage}
% \begin{minipage}{0.47\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_4.eps}
% \\ (\romannumeral4)
% \end{minipage}
\caption{Diagrams of Drell-S${\rm \ddot{o}ding}$ $\pi^{+}\pi^{-}$ production: (left and middle) dominant diagrams corresponding to $\pi^+-$nucleus and $\pi^--$nucleus scattering; (right) $\pi^+\pi^--$nucleus coupling diagram}
\label{fig:1}
\end{figure}
\DIFaddend %The wavy structures represent local energy fluctuations, while the blue and red virtual particle pairs depict short-lived quantum vacuum fluctuations in the electromagnetic field.

% Data detector and trigger

The measurement of exclusive $\pi^{+}\pi^{-}$ production \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend conducted in Au+Au UPCs at $\sqrt{s_{NN}}=200$ GeV at the Relativistic Heavy Ion Collider (RHIC) using the Solenoidal Tracker at RHIC (STAR)~\cite{STAR:detector}. An inclusive UPC trigger \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend applied for the pre-selection to the data~\cite{star:trigger}. This \DIFdelbegin \DIFdel{UPC trigger relies }\DIFdelend \DIFaddbegin \DIFadd{trigger relied }\DIFaddend on rapidity gaps defined by the small beam-beam counter (BBC) tiles on both sides \DIFaddbegin \DIFadd{of the detector }\DIFaddend ($3<\eta<5$)~\cite{star-bbc1,star:bbc2}, low activity in the mid-rapidity in the barrel time-of-flight (TOF) system~\cite{star:tof,Chen:2024aom} (TOF multiplicity between 1 and 7), and the coincidence of neutrons hitting both the east and west zero degree calorimeters (ZDC)~\cite{star:zdc,Xu:2016alq}. \DIFdelbegin \DIFdel{We analyze a total of 135 million triggered events collected in 2010, 2011, and 2014. }\DIFdelend The integrated luminosities for the triggered \DIFdelbegin \DIFdel{datasets }\DIFdelend \DIFaddbegin \DIFadd{data sets }\DIFaddend recorded in 2010, 2011, and 2014 are 679\DIFdelbegin \DIFdel{$\pm$ 68}\DIFdelend , 859\DIFdelbegin \DIFdel{$\pm$ 86}\DIFdelend , and 1464 \DIFdelbegin \DIFdel{$\pm$ 146 }\DIFdelend $\mu b^{-1}$ \DIFaddbegin \DIFadd{with 10\% uncertainty}\DIFaddend , respectively. The momenta of charged-particle tracks \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend reconstructed by the time projection chamber (TPC) covering pseudorapidities $\vert \eta \vert<1.0$ for the full azimuthal angle ($0<\phi<2\pi$)~\cite{star:tpc}. %The TPC also provides the specific ionization loss (dE/dx) measurement for the particle identification of each tracks.
The TPC also \DIFdelbegin \DIFdel{provides }\DIFdelend \DIFaddbegin \DIFadd{provided }\DIFaddend specific ionization energy loss (dE/dx) measurements for particle identification, which \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend used to construct the deviation parameter $n\sigma_\pi$ by comparing the measured dE/dx to the value predicted for a pion.


Further offline \DIFdelbegin \DIFdel{selections are }\DIFdelend \DIFaddbegin \DIFadd{cuts on the events were }\DIFaddend required. Events \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend required to have a primary vertex reconstructed by a pair of charged-particle tracks with a longitudinal distance of $\vert V_z \vert<100$ cm to the nominal center of STAR. The associated charged-particle tracks \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend required to have at least 15 fit points and 10 dE/dx points to ensure sufficient momentum and dE/dx resolutions. Charged-particle tracks \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend required to match to TOF hits \DIFaddbegin \DIFadd{in order }\DIFaddend to mitigate the effect of out-of-time pileup. The distance of closest approach (DCA) for charged-particle tracks \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend required to be less than 1.5 cm to the primary collision vertex to suppress contamination by secondary decay particles. High purity $\pi^{+}\pi^{-}$ pairs \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend selected by requiring $\chi^2_{\pi\pi}=n\sigma_{\pi 1}^2+n\sigma_{\pi 2}^2<8$, which \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend almost fully efficient ($\sim99\%$). 
\DIFdelbegin \DIFdel{The azimuthal decay }\DIFdelend %DIF > The azimuthal decay angle $\Delta\phi$ is calculated as $\Delta\phi = \phi_{\pi} - \phi_{\text{pair}}$, where $\phi_{\pi}$ is the azimuthal angle of the $\pi^+$ or $\pi^-$ in the $\pi^+\pi^-$ rest frame and $\phi_{\text{pair}}$ is the azimuthal angle of the pair momentum in the laboratory frame. 
\DIFaddbegin \DIFadd{The azimuthal }\DIFaddend angle $\Delta\phi$ is \DIFdelbegin \DIFdel{calculated as $\Delta\phi = \phi_{\pi} - \phi_{\text{pair}}$, where $\phi_{\pi}$ is the azimuthal angle }\DIFdelend \DIFaddbegin \DIFadd{defined in the transverse plane as the angle between $\vec{p}_{T1}+\vec{p}_{T2}$ and $\vec{p}_{T1}-\vec{p}_{T2}$, where $\vec{p}_{T1}$ and $\vec{p}_{T2}$ are the transverse momenta }\DIFaddend of the
$\pi^+$ \DIFdelbegin \DIFdel{or }\DIFdelend \DIFaddbegin \DIFadd{and }\DIFaddend $\pi^-$\DIFdelbegin \DIFdel{in the $\pi^+\pi^-$ rest frame and $\phi_{\text{pair}}$ is the azimuthal angle of the pair momentum in the laboratory frame}\DIFdelend .
Over one million exclusive $\pi^{+}\pi^{-}$ pairs \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend selected in the invariant mass region $0.6<M_{\pi^+\pi^-}<0.9$ GeV/${\rm c^2}$, enabling precise differential spectra studies.

% embedding and efficiency correction
A Monte Carlo (MC) sample \DIFdelbegin \DIFdel{is generatedwith $V_z$ distributions }\DIFdelend \DIFaddbegin \DIFadd{of photoproduced $\pi^+\pi^-$ pairs was generated. The kinematic distributions were weighted according to the model described in Ref.~\mbox{%DIFAUXCMD
\cite{Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
. The vertex ($V_z$) distribution was }\DIFaddend matched to data. The sample \DIFdelbegin \DIFdel{passes }\DIFdelend \DIFaddbegin \DIFadd{data was passed }\DIFaddend through the STAR detector response \DIFdelbegin \DIFdel{simulation based on }\DIFdelend \DIFaddbegin \DIFadd{simulator using }\DIFaddend GEANT3~\cite{Brun:1119728} to evaluate the acceptance and detector efficiency. It \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend then embedded into randomly recorded STAR events that \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend tuned to reproduce the ZDC \DIFdelbegin \DIFdel{confidence }\DIFdelend \DIFaddbegin \DIFadd{coincidence }\DIFaddend rate during data taking, ensuring realistic background effects on charged-particle track and vertex reconstruction. To \DIFdelbegin \DIFdel{reduce the model dependence}\DIFdelend \DIFaddbegin \DIFadd{minimize potential biases arising from the Monte Carlo sample's underlying kinematic distributions}\DIFaddend , a high-dimensional correction \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend employed to obtain the cross section as
\begin{equation}
    \frac{d^3 \sigma}{d p_T d M d \Delta \phi} =\frac{N\left(p_T, M, \Delta \phi\right)}{\varepsilon_{\text {trig }}{\text{corr}}(p_T, M, \Delta \phi)L\Delta p_T\Delta M\Delta(\Delta \phi)},
\end{equation}
where $\varepsilon_{\text {trig }}$ is the trigger efficiency; $\text{corr}(p_T, M, \Delta \phi)$ represents the $p_T$, $M$, and $\Delta \phi$-dependent acceptance and efficiency correction; and $L$ is the integrated luminosity. Since signals \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend corrected with the $\Delta \phi$ dependence, the amplitudes of the $\Delta \phi$ modulations at all orders \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend corrected simultaneously. In addition, the momentum smearing of charged-particle tracks in \DIFaddbegin \DIFadd{the }\DIFaddend TPC smooths the $\Delta \phi$ spectra, especially at low $\pi^{+}\pi^{-}$ $p_T$. We \DIFdelbegin \DIFdel{estimate }\DIFdelend \DIFaddbegin \DIFadd{estimated }\DIFaddend the momentum resolution impact and unfold the measured ${\rm A_{2\Delta\phi}}$ based on the ratio of the reconstructed ${\rm A_{2\Delta\phi}}$ to the original in the polarized Monte Carlo simulation\DIFaddbegin \DIFadd{, where the $\Delta\phi$ distribution was reweighted according to the polarization model}\DIFaddend .
% different processes separation (mass fitting)

\DIFdelbegin \begin{displaymath}
\DIFdel{\begin{aligned}
\frac{d \sigma}{d M_{\pi^{+} \pi^{-}}} &= \left| A_\rho \frac{\sqrt{M_{\pi \pi} M_{\rho} \Gamma_\rho}}{M_{\pi \pi}^2-M_\rho^2+i M_\rho \Gamma_\rho} f_{fluxcorr} + B f_{S\ddot{o}ding} \right. \\ 
&\left. + C_\omega e^{i \phi_\omega} \frac{\sqrt{M_{\pi \pi} M_\omega \Gamma_{\omega \rightarrow \pi \pi}}}{M_{\pi \pi}^2-M_\omega^2+i M_\omega \Gamma_\omega} \right|^2 + f_{\mu\mu} + f_{\text {bg}}.
\end{aligned}
%DIFDELCMD < \label{eq:fit}%%%
}\end{displaymath}%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend An improved description of the exclusive $\pi^{+}\pi^{-}$ mass distribution \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend constructed to separate the resonance and non-resonance components from different processes, as expressed in Eq.~\ref{eq:fit}. In this parameterization, $A_\rho$ and $C_\omega$ denote the amplitudes for $\rho^0$ and $\omega$, respectively; $B$ represents the magnitude of the normalized model-calculated Drell-S${\rm \ddot{o}ding}$ mass shape $f_{S\ddot{o}ding}$; \DIFdelbegin \DIFdel{and }\DIFdelend $\phi_\omega$ is the mixing phase angle for $\omega$\DIFaddbegin \DIFadd{; and $f_{\text {bg}}$ is a linear polynomial that accounts for any residual non-photoproduction background}\DIFaddend . We apply the relativistic Breit-Wigner (rBW) resonance for $\rho^0$ and $\omega$, and a phenomenological non-resonance by the NRP calculation\DIFaddbegin \DIFadd{~\mbox{%DIFAUXCMD
\cite{Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend . The momentum-dependent mass widths are expressed as~\cite{Alvensleben:1971hz}
% Fitting mass figure
\begin{equation}
\begin{aligned}
&\Gamma_\rho=\Gamma_0 \frac{M_\rho}{M_{\pi \pi}}\left(\frac{M_{\pi \pi}^2-4 m_\pi^2}{M_\rho^2-4 m_\pi^2}\right)^{3 / 2},\\
&\Gamma_{\omega \rightarrow \pi \pi}=\operatorname{Br}(\omega \rightarrow \pi \pi) \Gamma_0 \frac{M_\omega}{M_{\pi \pi}}\left(\frac{M_{\pi \pi}^2-4 m_\pi^2}{M_\omega^2-4 m_\pi^2}\right)^{3 / 2},
\end{aligned}
\end{equation}
with $\operatorname{Br}(\omega \rightarrow \pi \pi)=0.0153^{+0.0011}_{-0.0013}$~\cite{ParticleDataGroup:2014cgo}, where $\Gamma_0$ is the pole \DIFdelbegin \DIFdel{meson width }\DIFdelend \DIFaddbegin \DIFadd{width for each meson}\DIFaddend . 
The vector meson photoproduction amplitude \DIFdelbegin \DIFdel{could be }\DIFdelend \DIFaddbegin \DIFadd{is }\DIFaddend modeled as the photon energy distribution and scattering amplitude for the virtual vector meson and nucleus. Due to the correlation of the photon energy and vector meson mass, $E_{\gamma}=M/2\times exp(\pm y)$, the photon energy distribution \DIFdelbegin \DIFdel{would }\DIFdelend slightly modify the rBW mass spectra. This correction, $f_{fluxcorr}$, is considered using VMD model calculation~\cite{PhysRevD.103.033007,Zha:2018jin}. The $\gamma\gamma \rightarrow \mu^+ \mu^-$ process constitutes a \DIFdelbegin \DIFdel{non-negligible }\DIFdelend background, as muons cannot be distinguished from pions due to the absence of a start time $t_0$ measurement for TOF. Dimuon production, $f_{\mu\mu}$, is calculated using lowest-order QED~\cite{Li:2023yjt,Zha:2018tlq,Zha:2021jhf}, which \DIFdelbegin \DIFdel{has been demonstrated to describe the experimental measurement well}\DIFdelend \DIFaddbegin \DIFadd{reproduces experimental data}\DIFaddend ~\cite{STAR:2018ldd,STAR:2019wlg}.


\DIFaddbegin \begin{equation}
\DIFadd{\begin{aligned}
\frac{d \sigma}{d M_{\pi^{+} \pi^{-}}} &= \left| A_\rho \frac{\sqrt{M_{\pi \pi} M_{\rho} \Gamma_\rho}}{M_{\pi \pi}^2-M_\rho^2+i M_\rho \Gamma_\rho} f_{fluxcorr} + B f_{S\ddot{o}ding} \right. \\ 
&\left. + C_\omega e^{i \phi_\omega} \frac{\sqrt{M_{\pi \pi} M_\omega \Gamma_{\omega \rightarrow \pi \pi}}}{M_{\pi \pi}^2-M_\omega^2+i M_\omega \Gamma_\omega} \right|^2 + f_{\mu\mu} + f_{\text {bg}}.
\end{aligned}
\label{eq:fit}
}\end{equation}
\DIFaddend %Where $A_\rho$ and $C_\omega$ are the amplitudes for $\rho^0$ and $\omega$, respectively. The $\phi_\omega$ is the mixing phase angle for $\omega$. The momentum-dependent mass widths are expressed as~\cite{Alvensleben:1971hz}
% Fitting mass figure


\DIFdelbegin %DIFDELCMD < \begin{figure}[h]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.495\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{mass_fit_tot_run10_0.6_1.3_11_10_25.eps}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{The differential cross section $d^2\sigma/dM_{\pi\pi}dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $p_T<0.1$ GeV/c and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV, together with illustration of the fitting algorithm to separate resonance and continuum components. The black markers show the data, and the lilac markers show the Drell-S${\rm \ddot{o}ding}$ term. The interference terms for $\rho$-Söding (purple), $\omega$-Söding (brown), and $\rho-\omega$ (dark green) are shown. $\mu^+\mu^-$ pair production is represented by the blue band.}
%DIFDELCMD <   \label{fig:2}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \begin{figure}[h]
  \centering
  \begin{minipage}{0.495\textwidth}
    \includegraphics[width=\textwidth]{GPCreviewfigure/mass_fit_tot_run10_0.6_1.3_4_6_26.eps}
  \end{minipage}
   \caption{The differential cross section $d^2\sigma/dM_{\pi\pi}dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $p_T<0.1$ GeV/c and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV, together with an illustration of the fitting algorithm to separate the $\rho^{0}$ and Drell-S${\rm \ddot{o}ding}$ components. The black markers show the data, and the lilac line show the Drell-S${\rm \ddot{o}ding}$ term. The interference terms for $\rho$-Söding (purple), $\omega$-Söding (brown), and $\rho-\omega$ (dark green) are shown. $\mu^+\mu^-$ pair production is represented by the blue band.}
  \label{fig:2}
\end{figure}
\DIFaddend 


\DIFdelbegin %DIFDELCMD < \begin{figure}[h]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.48\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{GPCreviewfigure/paper_dt_ratio_theocomp_mass0609.eps}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{(top) The differential cross section $d\sigma/d|t|dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $0.6<M<0.9$ GeV/${\rm c^2}$ and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. The blue and red markers (lines) represent the measured (calculated) $\rho^0$ photoproduction~\cite{Zha:2018jin} and Drell-S${\rm \ddot{o}ding}$ process~\cite{pumplin1970diffraction,bolz2015photoproduction}, respectively. (bottom) The measured (calculated) ratio of the Drell-S${\rm \ddot{o}ding}$ to $\rho^0$ photoproduction cross sections provides insight into the photon’s hadronic structure and indicates a softer production mechanism.}
%DIFDELCMD <   \label{fig:3}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \begin{figure}[h]
  \centering
  \begin{minipage}{0.48\textwidth}
    \includegraphics[width=\textwidth]{GPCreviewfigure/paper_dt_ratio_theocomp_mass0609.eps}
  \end{minipage}
   \caption{(top) The differential cross section $d^{2}\sigma/d|t|dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $0.6<M<0.9$ GeV/${\rm c^2}$ and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. The blue and red markers (lines) represent the measured (calculated) $\rho^0$ photoproduction~\cite{Zha:2018jin} and Drell-S${\rm \ddot{o}ding}$ process~\cite{pumplin1970diffraction,bolz2015photoproduction,Wu:2026emu}, respectively. EPA denotes the equivalent photon approximation. (bottom) The measured (calculated) ratio of the Drell-S${\rm \ddot{o}ding}$ to $\rho^0$ photoproduction cross sections.} 
   %provides insight into the photon’s hadronic structure and indicates a softer production mechanism.}
  \label{fig:3}
\end{figure}
\DIFaddend %The theoretical calculation, however, does not reproduce the measured trend.
%DIF < The Drell-S${\rm \ddot{o}ding}$ term is represented by a normalized model-calculated mass shape $f_{S\ddot{o}ding}$, scaled by a free parameter $B$ that reflects its magnitude. 
%DIF < Correction for the rBW $\rho^0$ induced by the photon energy distribution is considered by the VMD model calculation as $f_{fluxcorr}$~\cite{PhysRevD.103.033007,Zha:2018jin}. The vector meson photoproduction amplitude could be modeled as the photon energy distribution and scattering amplitude for the virtual vector meson and nucleus. Due to the correlation of the photon energy and vector meson mass, $E_{\gamma}=M/2\times exp(\pm y)$, the photon energy distribution would slightly modify the rBW mass spectra. Dimuon production is calculated using lowest-order QED~\cite{Li:2023yjt,Zha:2018tlq,Zha:2021jhf}, incorporating both parallel and cross diagrams, which has been demonstrated to describe the experimental measurement well~\cite{STAR:2018ldd,STAR:2019wlg}.

\DIFdelbegin %DIFDELCMD < \begin{figure*}[ht]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.96\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{paper_a2_pt_mass_11_7_25.eps}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{The second order modulation amplitude $A_{2\Delta\phi}$ as functions of the pair transverse momentum $p_T$ (left) and the invariant mass $M_{\pi^+\pi^-}$ (right) for $0<p_T<0.1$ GeV/c, $0.6<M_{\pi^+\pi^-}<0.9$ GeV/${\rm c^2}$, and $\vert y \vert<0.9$ in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV. The Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction are shown in red and teal points. Statistic uncertainties and systematic uncertainties are represented by the error bars and boxes (left), or band (right) respectively. The model calculations are donated as dash lines.}
%DIFDELCMD <   \label{fig:4}
%DIFDELCMD < \end{figure*}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \begin{figure*}[ht]
  \centering
  \begin{minipage}{0.96\textwidth}
    \includegraphics[width=\textwidth]{GPCreviewfigure/paper_a2_pt_mass_4_2_26.eps}
  \end{minipage}
   \caption{The $\Delta\phi$ distributions normalized to unit integral (left); second-order modulation amplitude $A_{2\Delta\phi}$ versus pair transverse momentum $p_T$ (middle) and invariant mass $M_{\pi^+\pi^-}$ (right) in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV. The Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction data points are shown as red and teal points. Statistical uncertainties and systematic uncertainties are represented by the error bars and boxes (middle), or bands (left and right) respectively. The model calculations are denoted as dashed lines. In the middle panel, the data and model calculations use the same binning in $p_T$. For clarity, the $\rho^0$ and Drell–S${\rm \ddot{o}ding}$ data points are slightly shifted horizontally relative to the bin centers to avoid overlap.}
  \label{fig:4}
\end{figure*}
\DIFaddend 

%DIF > The correlated uncertainties are estimated to be 2% and 5% of the extracted yields for $\rho^0$ and Drell-Söding
%Systematic uncertainty
Systematic uncertainties are classified into correlated and uncorrelated components \DIFaddbegin \DIFadd{among different data sets}\DIFaddend . Correlated uncertainties \DIFdelbegin \DIFdel{, }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend estimated to be 2\% for $\rho^0$ and 5\% for Drell-Söding, \DIFdelbegin \DIFdel{arise }\DIFdelend \DIFaddbegin \DIFadd{arising }\DIFaddend mainly from the fitting procedure, including \DIFdelbegin \DIFdel{the choice }\DIFdelend \DIFaddbegin \DIFadd{choices }\DIFaddend of fitting range and the modeling of the Drell-S${\rm \ddot{o}ding}$ mass shape. The \DIFdelbegin \DIFdel{fitting stability is }\DIFdelend \DIFaddbegin \DIFadd{fitting-range dependence was }\DIFaddend evaluated by varying the \DIFdelbegin \DIFdel{lower }\DIFdelend \DIFaddbegin \DIFadd{low }\DIFaddend mass boundary from 0.6 GeV/${\rm c^2}$ to 0.57 GeV/${\rm c^2}$ and 0.65 GeV/${\rm c^2}$.
An alternative parametrization of the non-resonant amplitude, $A_{nr}= f_{nr}/(m_{\pi\pi}^2-4m_\pi^2+\Lambda_{nr}^2)^{\delta_{nr}}$, following Ref.~\cite{H1:2020lzc}, \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend used to assess the model dependence \DIFdelbegin \DIFdel{. }\DIFdelend \DIFaddbegin \DIFadd{of the fit to the data, }\DIFaddend where $f_{n r}$, $\Lambda_{n r}$, and $\delta_{n r}$ are free parameters. 
%While this approach enhances model flexibility, it introduces sensitivity to local minima during the fitting process.
Uncorrelated uncertainties \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend evaluated through variations in topological selection criteria and adjustments to the MC model in acceptance and efficiency extractions. Uncorrelated uncertainties are about 5\% for $\rho^0$ photoproduction and 8\% for Drell-S${\rm \ddot{o}ding}$. An external 10\% uncertainty in integrated luminosity determination and a 3\% per-track reconstruction uncertainty are included. 
Results from different \DIFdelbegin \DIFdel{datasets }\DIFdelend \DIFaddbegin \DIFadd{data sets }\DIFaddend are statistically consistent within uncertainties and are combined using a weighted average based on the quadratic sum of statistical and uncorrelated systematic uncertainties. The \DIFaddbegin \DIFadd{statistical and uncorrelated systematic uncertainties are treated as independent and are propagated to the combined result by summing their contributions in quadrature with the corresponding weights.
The correlated systematic uncertainties, assumed to be fully correlated across data sets, are combined by taking their weighted average.
The correlations between $\rho^0$ photoproduction and Drell-S${\rm \ddot{o}ding}$ are accounted for through the covariance matrix in the fit.
The }\DIFaddend total systematic uncertainty is obtained by \DIFdelbegin \DIFdel{combining }\DIFdelend \DIFaddbegin \DIFadd{adding }\DIFaddend the uncorrelated and correlated uncertainties in quadrature. 
%DIF < The results of each dataset are consistent within uncertainties and combined with the weight using the statistic uncertainties and uncorrelated systematic uncertainties.
\DIFaddbegin \DIFadd{The systematic uncertainty sources and evaluation procedure are the same for the extracted $A_{2\Delta\phi}$. For the difference between the $A_{2\Delta\phi}$ of $\rho^0$ and Drell-S${\rm \ddot{o}ding}$, the uncertainty is evaluated directly on the difference, such that the correlations between them are naturally included.
%DIF > The results of each data set are consistent within uncertainties and combined with the weight using the statistic uncertainties and uncorrelated systematic uncertainties.
}\DIFaddend %\begin{equation}
%    \begin{aligned}
        %&w_i = \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}/W,\\ \text{where} \ &W=\sum_i \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}.
%        w_i = \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}/(\sum_i \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}).
%    \end{aligned}
%\end{equation}
%The total systematic uncertainty is obtained by combining the uncorrelated and correlated uncertainties in quadrature.


Figure~\ref{fig:2} illustrates the differential cross section $d^2\sigma/dM_{\pi\pi}dy$ as a function of the invariant mass $M_{\pi\pi}$.
%in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. 
The data points represent the measured cross section, while the red curve shows the full fit incorporating various contributing components.
%DIF < The dominant $\rho^0$ rBW accounts for the primary resonance structure, with additional contributions from the $\omega$ rBW component and the Drell-Söding process. The interference terms, including $\rho$-Söding, $\omega$-Söding, and $\omega$-$\rho$ interference, modulate the overall shape. The shaded blue region represents the background from $\gamma\gamma \rightarrow \mu^+\mu^-$ process. The enhancement of the cross section of $\gamma\gamma \rightarrow \mu^+\mu^-$ by setting the $\mu$ tracks with the $\pi$ mass is considered in QED calculations.
%DIF < addsomething here 1 DS is a small contribution however we could still precise measure it due to the key role for the interference in determining the cross section 
Although the Drell-S${\rm \ddot{o}ding}$ process constitutes a relatively minor contribution to exclusive $\pi^+\pi^-$ production, its interference with the $\rho^0$ production crucially shapes the observed mass spectrum. The mass shift and the asymmetric structure of the mass peak are both governed by this interference thus enabling a precise extraction of the Drell-Söding contribution. \DIFdelbegin \DIFdel{We perform mass fits per pair }\DIFdelend \DIFaddbegin \DIFadd{Mass spectra are fitted independently in each (}\DIFaddend $p_T$\DIFdelbegin \DIFdel{and }\DIFdelend \DIFaddbegin \DIFadd{, }\DIFaddend $\Delta \phi$\DIFdelbegin \DIFdel{to disentangle the differential cross section for each process.
}\DIFdelend \DIFaddbegin \DIFadd{) bin to extract the contributions of the different processes and evaluate the corresponding cross sections..
%DIF > We perform mass fits per pair $p_T$ and $\Delta \phi$ to disentangle the differential cross section for each process.
}\DIFaddend %Although the Drell-S${\rm \ddot{o}ding}$ process accounts for a relatively small contribution of the exclusive $\pi^+\pi^-$ production, the interference of the Drell-S${\rm \ddot{o}ding}$ and $\rho^0$ production plays a key role in shaping the mass spectrum. 
%DIF < The fact that the mass shift and the shape of both sides of the mass peak are determined by the interference effect between the Drell-S${\rm \ddot{o}ding}$ and $\rho^0$ production ensures the feasibility of precisely measuring the Drell-Söding process. We perform mass fits per pair $p_T$ and $\Delta \phi$ to measure the differential cross section for each process. 
Amplitudes of the second order cosine modulation ${\rm A_{2\Delta\phi}}$ could be reconstructed by a weighted sum ${\rm A_{2\Delta\phi}}=\sum_{i=1}^n 2N_i{\rm cos(2\Delta \phi_i)}$, %DIF > where $N_i$ is the normalized yield at $\Delta \phi_i$. 
where $N_i$ \DIFdelbegin \DIFdel{is the normalized yield at }\DIFdelend \DIFaddbegin \DIFadd{denotes the yield in each }\DIFaddend $\Delta \phi_i$ \DIFdelbegin \DIFdel{. 
%DIF < The quality of the fits is quantified by the reduced chi-square, $\chi^2/\text{ndf}$, which ranges from 50 to 100 per 65 degrees of freedom ($50/65\sim100/65$) for mass fits performed in different $p_T$, $\Delta\phi$ and $p_T-\Delta\phi$ bins.
}\DIFdelend \DIFaddbegin \DIFadd{bin normalized by the total yield in the corresponding $p_T$ interval.
}\DIFaddend The fit quality is evaluated using the reduced chi-square ($\chi^2/\text{ndf}$), which ranges from 50 to 100 per 65 degrees of freedom, reflecting consistent modeling of the spectral features.


%Fig.~\ref{fig:3} shows the differential cross section $d^2\sigma/dp_T^2dy$ for Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction with their ratio on the pair $p_T$ dependence. The Drell-S${\rm \ddot{o}ding}$ exhibit a sharper decreasing slope with $p_T$ increase and an obviously smaller $p_T$ for the diffractive dips which are related to the nucleus imaging. The ratio shows a significant bump which definitively demonstrate Drell-S${\rm \ddot{o}ding}$ process is softer than the $\rho^0$ production although they are both $\gamma A \rightarrow \pi^+\pi^-A$ processes. The results indicate the photon hadronic structure that the virtual $\pi^+\pi^-$ pair fluctuation concentrate more at lower photon energy region compared to virtual $\rho^0$.

% gpt improved:
Figure~\ref{fig:3} presents the differential cross-section $d^2\sigma/d|t| dy$ for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction, along with their ratio as a function of \DIFdelbegin \DIFdel{$|t|$}\DIFdelend \DIFaddbegin \DIFadd{$|t| \approx p_{T\pi^{+}\pi^{-}}^{2}$}\DIFaddend . The $\rho^0$ results are consistent with the previous measurement~\cite{STAR:2017enh}.
%DIF < The Drell-S${\rm \ddot{o}ding}$ process exhibits a steeper decline with increasing $p_T$ compared to $\rho^0$ photoproduction, with a noticeably lower $p_T$ position for the diffractive minima, which are associated with nuclear imaging. 
Compared to $\rho^0$ photoproduction, the Drell-S${\rm \ddot{o}ding}$ process exhibits a steeper decline with increasing $|t|$ with its diffractive minima shifted to lower $|t|$, reflecting a softer production mechanism and differences in the underlying photon hadronic structure.
The measured ratio reveals a pronounced bump at low $|t|$, suggesting that the virtual $\pi^+\pi^-$ configuration is spatially broader than the $\rho^0$ state. Theoretical calculations do not reproduce this trend, possibly due to missing dipole-size effects that are not accounted for in the model.

Figure~\ref{fig:4} shows the azimuthal anisotropy \DIFaddbegin \DIFadd{(left)}\DIFaddend , quantified by the second-order cosine modulation amplitude, ${\rm A_{2\Delta\phi}}$, for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction as functions of the pair transverse momentum $p_T$ (\DIFdelbegin \DIFdel{left}\DIFdelend \DIFaddbegin \DIFadd{middle}\DIFaddend ) and the invariant mass $M_{\pi^+\pi^-}$ (right) within rapidity $|y|<0.9$. The amplitudes, ${\rm A_{2\Delta\phi}}$, are determined by performing invariant mass fits in distinct $\Delta\phi$ or $p_T$-vs-$\Delta\phi$ intervals. To ensure sufficient statistical precision for resolving subtle features in the mass distribution, the $p_T$ range is divided into three bins: $0 < p_T < 0.03~\mathrm{GeV}/c$, $0.03 < p_T < 0.05~\mathrm{GeV}/c$, and $0.05 < p_T < 0.1~\mathrm{GeV}/c$. The resulting \DIFdelbegin \DIFdel{differential cross section as a function of }\DIFdelend $\Delta\phi$ \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{distributions are }\DIFaddend then used to extract the $\cos(2\Delta\phi)$ modulation amplitude. 
%DIF < Fig.~\ref{fig:4} presents the azimuthal anisotropy quantified by the amplitude of the second order cosine modulation $A_{2\Delta\phi}$ for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction as functions of the pair transverse momentum $p_T$ (left) and the invariant mass $M_{\pi^+\pi^-}$ (right) for rapidity $|y|<0.9$. In order to measure the amplitudes $A_{2\Delta\phi}$, the mass fits are performed in different $\Delta\phi$ or $p_T-\Delta\phi$ intervals. The pair $p_T$ is divided into three bins as $0<p_T<0.03$ GeV/c, $0.03<p_T<0.05$ GeV/c and $0.05<p_T<0.1$ GeV/c for the differential mass fits in $p_T-\Delta\phi$ intervals. This is to guarantee enough statistics for a series of good fits to the subtle mass shape. Consequently, the obtained differential cross section as a function of $\Delta\phi$ is used to reconstruct the amplitude of $cos(2(\Delta\phi))$ modulation. The mass dependence of the amplitude $A_{2\Delta\phi}$ in an integrated pair transverse momentum $0<p_T<0.1$ GeV/c is presented in the right figure.
The ${\rm A_{2\Delta\phi}}$ of the Drell-S${\rm \ddot{o}ding}$ process exhibits a similar $p_T$ dependence \DIFdelbegin \DIFdel{with the }\DIFdelend \DIFaddbegin \DIFadd{as }\DIFaddend $\rho^0$ photoproduction and \DIFaddbegin \DIFadd{has }\DIFaddend an enhancement in transverse momentum in the range $0.05<p_T<0.1$ GeV/c. 
%DIF < For exclusive $\pi^+\pi^-$ production, the yield in this $p_T$ intervals constitutes about half of the yield over $0<p_T<0.1$ GeV/c. The Drell-S${\rm \ddot{o}ding}$ is known to have a softer $p_T$ distribution compared to $\rho^0$ from Fig.~\ref{fig:3}. 
The right panel illustrates the $M_{\pi^+\pi^-}$ dependence of ${\rm A_{2\Delta\phi}}$\DIFdelbegin \DIFdel{integrated over the full $p_T$ range, $0 < p_T < 0.1~\mathrm{GeV}/c$. 
The $A_{2\Delta\phi}$ is found to have a relatively flat }\DIFdelend \DIFaddbegin \DIFadd{. 
%DIF > integrated over the full $p_T$ range, $0 < p_T < 0.1~\mathrm{GeV}/c$. 
%DIF > The ${\rm A_{2\Delta\phi}}$ is found to have a relatively flat $M_{\pi^+\pi^-}$ dependence
No significant }\DIFaddend $M_{\pi^+\pi^-}$ dependence \DIFdelbegin \DIFdel{, suggesting minimal }\DIFdelend \DIFaddbegin \DIFadd{of ${\rm A_{2\Delta\phi}}$ is found, indicating no strong }\DIFaddend photon energy dependence in EESI. Notably, the \DIFdelbegin \DIFdel{measured }\DIFdelend \DIFaddbegin \DIFadd{extracted }\DIFaddend ${\rm A_{2\Delta\phi}}$ for the Drell-S${\rm \ddot{o}ding}$ \DIFaddbegin \DIFadd{process }\DIFaddend is systematically higher than that for $\rho^0$ photoproduction.
\DIFdelbegin \DIFdel{When integrated over }\DIFdelend \DIFaddbegin \DIFadd{For $0 < p_T < 0.1~\mathrm{GeV}/c$, $|y| < 0.9$, and }\DIFaddend $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$, \DIFdelbegin \DIFdel{the difference corresponds to a significance of 4.6~$\sigma$, evaluated including all statistical and systematic uncertainties. Specifically, }\DIFdelend \DIFaddbegin \DIFadd{the extracted }\DIFaddend ${\rm A_{2\Delta\phi}}$ values \DIFdelbegin \DIFdel{for $0 < p_T < 0.1~\mathrm{GeV}/c$, $|y| < 0.9$ and $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$ are measured as $0.2702 \pm 0.0024 \pm 0.0120$ }\DIFdelend \DIFaddbegin \DIFadd{are $0.273 \pm 0.010 \pm 0.013$ }\DIFaddend (Drell-S${\rm \ddot{o}ding}$) and \DIFdelbegin \DIFdel{$0.2181 \pm 0.0022 \pm 0.0050$ }\DIFdelend \DIFaddbegin \DIFadd{$0.219 \pm 0.003 \pm 0.005$ }\DIFaddend ($\rho^0$ photoproduction). The first quoted errors are statistical uncertainties\DIFaddbegin \DIFadd{, }\DIFaddend while the second are \DIFdelbegin \DIFdel{systematical uncertainties. %DIF < Notably, the measured ${\rm A_{2\Delta\phi}}$ as a function of $M_{\pi^+\pi^-}$ for the Drell-S${\rm \ddot{o}ding}$ in $0 < p_T < 0.1~\mathrm{GeV}/c$ is systematically higher than that for $\rho^0$ photoproduction. When integrated over $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$, the difference corresponds to a significance of $4.6\sigma$, evaluated including all statistical and systematic uncertainties. Specifically, ${\rm A_{2\Delta\phi}}$ values for $0 < p_T < 0.1~\mathrm{GeV}/c$, $|y| < 0.9$ and $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$ are measured as $0.2702 \pm 0.0024 \pm 0.0120$ (Drell-S${\rm \ddot{o}ding}$) and $0.2181 \pm 0.0022 \pm 0.0050$ ($\rho^0$ photoproduction). The first quoted errors are statistical uncertainties while the second are systematical uncertainties.
}\DIFdelend \DIFaddbegin \DIFadd{systematic uncertainties. The resulting difference is $0.054 \pm 0.010 \pm 0.015$, corresponds to a significance of 3.0~$\sigma$ when statistical and systematic uncertainties are included. 
}\DIFaddend 

The predictions of the EPA-VMD and NRP model are also compared with the data and found to \DIFdelbegin \DIFdel{understimate }\DIFdelend \DIFaddbegin \DIFadd{underestimate }\DIFaddend $A_{2\Delta\phi}$ at \DIFdelbegin \DIFdel{lower }\DIFdelend \DIFaddbegin \DIFadd{low }\DIFaddend transverse momentum, $0<p_T<0.05$ GeV/c. 
\DIFdelbegin \DIFdel{Based on the $A_{2\Delta\phi}$ measurement, specific contributions to the difference for the exclusive resonance and non-resonance produced entangled $\pi^+\pi^-$ pairs in cooperation with EESI can be studied. }\DIFdelend The results show no \DIFdelbegin \DIFdel{clear coherence lost in scattering with a nucleusand no clear destructive interference caused by the }\DIFdelend \DIFaddbegin \DIFadd{evidence, within the present uncertainties, for a loss of coherence in scattering off a nucleus, nor for destructive interference induced by the difference between the }\DIFaddend $\pi^+p$ and $\pi^-p$ scattering \DIFdelbegin \DIFdel{asymmetric }\DIFdelend amplitudes in the Drell-S${\rm \ddot{o}ding}$ process.
%DIF < It is also indicated no significant wave function collapse caused by the $\rho^0$ decay


% Final conclusion generated by DS
In conclusion, we report the observation of EESI in the Drell-S${\rm \ddot{o}ding}$ process and the pair $p_T$ and $M$ dependence of the differential cross section for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV at RHIC. A model-based Drell-S${\rm \ddot{o}ding}$ shape is employed to separate different processes involved in exclusive $\pi^+\pi^-$ production. 
%DIF < The Drell-S${\rm \ddot{o}ding}$ process is observed obviously softer from the pair $p_T$ spectrum compared to $\rho^0$ photoproduction. 
The observation of EESI effects demonstrates that the non-resonant $\pi^+\pi^-$ pairs are entangled in the Drell-S${\rm \ddot{o}ding}$ process. The amplitude, ${\rm A_{2\Delta\phi}}$, for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction are found to have similar decreasing trends along the pair $p_T$. Compared to \DIFaddbegin \DIFadd{the }\DIFaddend $\rho^0$, an enhancement is observed \DIFdelbegin \DIFdel{for }\DIFdelend \DIFaddbegin \DIFadd{in }\DIFaddend the Drell-S${\rm \ddot{o}ding}$ process \DIFdelbegin \DIFdel{for }\DIFdelend \DIFaddbegin \DIFadd{in }\DIFaddend pair $p_T$ in the range $0.05<p_T<0.1$ GeV/c. The measured ${\rm A_{2\Delta\phi}}$ for these processes is found to have no obvious pair mass $M_{\pi^+\pi^-}$ dependence, and the amplitude ${\rm A_{2\Delta\phi}}$ for Drell-S${\rm \ddot{o}ding}$ is \DIFdelbegin \DIFdel{4.6 }\DIFdelend \DIFaddbegin \DIFadd{3.0 }\DIFaddend $\sigma$ higher than for $\rho^0$ photoproduction \DIFdelbegin \DIFdel{among }\DIFdelend \DIFaddbegin \DIFadd{over }\DIFaddend the observed mass regions. Moreover, the observed Drell-S${\rm \ddot{o}ding}$ $|t|$ spectrum is softer when compared to $\rho^0$ photoproduction. \DIFdelbegin \DIFdel{A comprehensive analysis of the measurements is reported through the comparison between resonant and non-resonant $\pi^+\pi^-$ photoproduction. }\DIFdelend These results advance the exploration of quantum interference phenomena in photon–nucleus interactions, providing a basis for future investigations in ultraperipheral heavy-ion collisions.%DIF > A comprehensive analysis of the measurements is reported through the comparison between resonant and non-resonant $\pi^+\pi^-$ photoproduction. These results advance the exploration of quantum interference phenomena in photon–nucleus interactions, providing a basis for future investigations in ultraperipheral heavy-ion collisions.

%The exclusive $\pi^+\pi^-$ production can be measured as a probe to the nuclear gluon density and nuclear geometry. From the comparison between the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction, the photon hadronic structure by fluctuation to ($\rho^0$ and $\pi^+\pi^-$) and production mechanism could be studied with its impact on imaging the nucleus. 
%Acknowledgement
\DIFdelbegin \section*{\DIFdel{Acknowledgement}}
%DIFAUXCMD
\DIFdelend \DIFaddbegin 

\textit{\DIFadd{Acknowledgments}}\DIFadd{—}\DIFaddend We thank the RHIC Operations Group and SDCC at BNL, the NERSC Center at LBNL, and the Open Science Grid consortium for providing resources and support.  This work was supported in part by the Office of Nuclear Physics within the U.S. DOE Office of Science, the U.S. National Science Foundation, National Natural Science Foundation of China, Chinese Academy of Science, the Ministry of Science and Technology of China and the Chinese Ministry of Education, NSTC Taipei, the National Research Foundation of Korea, Czech Science Foundation and Ministry of Education, Youth and Sports of the Czech Republic, Hungarian National Research, Development and Innovation Office, New National Excellency Programme of the Hungarian Ministry of Human Capacities, Department of Atomic Energy and Department of Science and Technology of the Government of India, the National Science Centre and WUT ID-UB of Poland, German Bundesministerium f\"ur Bildung, Wissenschaft, Forschung and Technologie (BMBF), Helmholtz Association, Ministry of Education, Culture, Sports, Science, and Technology (MEXT), and Japan Society for the Promotion of Science (JSPS).
\DIFdelbegin %DIFDELCMD < \bibliography{reference}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin 

\bibliography{referencenew}
\DIFaddend 











==> instituional_diff_test_EESI_4_28_26.tex <==
%\label{sec:dataselection}

% physics：
% 1. mass ordering image the nucleus
% %%%% nuclear force (need pi N cross section)
% 2. novel probe for deep understanding the interference
% 3. comparason to rho:    
% how does different photon hadronic structure
% production mechanics
% affect imagining the nucleus and the interference


% Introduction:
% nuclear and vacuum structure
% photoproduction used for parton dis both sides
% Entanglement interference
% unsolved issue & It is of great interest to investigate...
% In this Letter, we present
% The data and the trigger
% Event track pid cut and observable recon
% 

%The vacuum under the extremely strong electromagnetic field produced in relativistic heavy ion collisions has a subtle partonic structure. The photon induced processes, vector meson photoproduction and photon photon process, have been extensively measured

%The extremely strong electromagnetic field generated in the relativistic heavy-ion collisions can be described as a co-moving photon cloud with beams~\cite{weizsacker1934ausstrahlung,williams1934nature}, and thus enables photon nuclear interactions~\cite{krauss1997photon}. In the scenario of such interactions, a photon fluctuates into a virtual vector meson or hadron-antihadron pair, which then scatters off the nucleus by Pomeron exchange (finite sum of gluon ladders). Therefore, photon-nuclear interactions provide a unique probe of the photon's hadronic structure~\cite{bauer1978hadronic,AbdulKhalek:2021gbh,Li:2022kwn} and serve as a complementary tool for studying key nuclear properties, including the nuclear gluon distributions~\cite{guzey2013exclusive} and the overall nuclear size~\cite{sciadv.abq3903,Klein:1999qj}.
Ultra-strong electromagnetic fields in relativistic heavy-ion collisions \DIFdelbegin \DIFdel{manifest }\DIFdelend \DIFaddbegin \DIFadd{are manifested }\DIFaddend as a comoving photon cloud accompanying the nuclei~\cite{weizsacker1934ausstrahlung,williams1934nature}, enabling photonuclear interactions. In these processes, a photon fluctuates into a virtual vector meson or hadron-antihadron pair, which scatters via Pomeron exchange (gluonic exchanges). Such interactions provide a unique probe of the photon's hadronic structure~\cite{bauer1978hadronic,AbdulKhalek:2021gbh,Li:2022kwn} and serve as a complementary tool for studying key nuclear properties, including nuclear gluon distributions~\cite{guzey2013exclusive} and the overall \DIFdelbegin \DIFdel{nuclear size }\DIFdelend \DIFaddbegin \DIFadd{size of the nucleus}\DIFaddend ~\cite{sciadv.abq3903,Klein:1999qj}.
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend %For a quasi-real photon with spin-1, dissociation processes must adhere to angular momentum conservation. The photon may fluctuate into either (\romannumeral1) a virtual vector meson, which retains the photon’s spin and parity quantum numbers $(J^{PC}=1^{--})$, or (\romannumeral2) a virtual hadron-antihadron pair, giving rise to non-resonant photoproduction, known as the Drell-S${\rm \ddot{o}ding}$ process. 
\DIFaddbegin 

\DIFaddend A quasi-real spin-1 photon can fluctuate into (\romannumeral1) a virtual vector meson $(J^{PC}=1^{--})$, or (\romannumeral2) a virtual hadron-antihadron pair, giving rise to non-resonant photoproduction, known as the Drell-S${\rm \ddot{o}ding}$ process. 
In the case of scalar mesons such as $\pi^{+}\pi^{-}$, the angular momentum is encoded in the pair orbital momentum, resulting in quantum entanglement between the $\pi^{+}$ and $\pi^{-}$ \DIFaddbegin \DIFadd{in the relative-motion spatial wave function}\DIFaddend . A separate quantum phenomenon arises from the collision geometry: since both nuclei can act as photon emitters or targets, the emission source (nucleus A or B) becomes \DIFdelbegin \DIFdel{almost }\DIFdelend indistinguishable, establishing a ``double-slit'' interference pattern at the femtometer scale~\cite{sciadv.abq3903,PhysRevD.103.033007}. This interference induces second-order cosine oscillations in the asymmetries of the decay angular $\Delta\phi$ distributions~\cite{xing2020cos}. \DIFdelbegin \DIFdel{In the Drell-S${\rm \ddot{o}ding}$ mechanism, }\DIFdelend %DIF > In the Drell-S${\rm \ddot{o}ding}$ mechanism, the relativistic $\pi^{+}\pi^{-}$ pair emerges via a photon-nuclear interaction and rapidly separates in nearly opposite directions. %at relativistic speeds.
\DIFaddbegin \DIFadd{In this picture, interference at the pair level arises from the indistinguishability of }\DIFaddend the \DIFdelbegin \DIFdel{relativistic }\DIFdelend \DIFaddbegin \DIFadd{photon emission sources, while the entanglement of the }\DIFaddend $\pi^{+}\pi^{-}$ \DIFdelbegin \DIFdel{pair emerges via photon-nuclear interaction and rapidly separates in nearly opposite directions. %DIF < at relativistic speeds. 
The pair resembles an Einstein-Podolsky-Rosen (EPR) system~\mbox{%DIFAUXCMD
\cite{Brandenburg:2024ksp} }\hspace{0pt}%DIFAUXCMD
with no further information transmission after production. 
It is of great interest to investigate in depth the interference and entanglement in the Drell-S${\rm \ddot{o}ding}$ process.
}%DIFDELCMD < 

%DIFDELCMD < %%%
%DIF < It is a chance to explore the effect of decay in comparison to the production with an intermediate state such as $\rho^0$. 
\DIFdelend \DIFaddbegin \DIFadd{final state allows this interference to manifest in the measured decay angular distributions, giving rise to EESI effect.
%DIF > As with all Einstein-Podolsky-Rosen (EPR) systems, it is of great interest to investigate in depth the interference and entanglement in the Drell-S${\rm \ddot{o}ding}$ process.
}\DIFaddend 

The \DIFdelbegin \DIFdel{Drell-S}\DIFdelend \DIFaddbegin \DIFadd{Drell–S}\DIFaddend ${\rm \ddot{o}ding}$ process \DIFaddbegin \DIFadd{is a sensitive probe of the nuclear gluon structure, nuclear gluon saturation, and shadowing effects~\mbox{%DIFAUXCMD
\cite{ZEUS:1997rof,Laget:2019tou}}\hspace{0pt}%DIFAUXCMD
.
It }\DIFaddend has two dominant diagrams\DIFdelbegin \DIFdel{through virtual $\pi^+/\pi^-$-nucleus scattering}\DIFdelend \DIFaddbegin \DIFadd{, corresponding to $\pi^+-$nucleus and $\pi^--$nucleus scattering~\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,bolz2015photoproduction}}\hspace{0pt}%DIFAUXCMD
, as }\DIFaddend depicted in Fig.~\ref{fig:1}. \DIFdelbegin \DIFdel{And another for the gauge invariance~\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,bolz2015photoproduction}}\hspace{0pt}%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{A sub-leading $\pi^+\pi^--$nucleus coupling diagram is included to ensure gauge invariance\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend .
In 1960, Drell first proposed \DIFdelbegin \DIFdel{the diagrams of this process as promising contributions }\DIFdelend \DIFaddbegin \DIFadd{these diagrams as promising contributors }\DIFaddend to secondary beams \DIFdelbegin \DIFdel{via the $\gamma \rightarrow \pi^+\pi^-$ process }\DIFdelend at SLAC~\cite{drell1960production}. Later in 1966, S${\rm \ddot{o}ding}$ \DIFdelbegin \DIFdel{calculated them }\DIFdelend \DIFaddbegin \DIFadd{carried out a full calculation of the $\gamma p \to \pi^+\pi^- p$ process and used it }\DIFaddend to explain the observed skewing of the $\rho^0$ resonance peak~\cite{soding1966apparent}. 
\DIFdelbegin \DIFdel{Compared to the resonance $\rho^0$, the direct $\pi^+\pi^-$ is more loosely bounded with a larger dipole size, corresponding to a smaller pair $p_T$ even at the same photon energy. With such a system scattering from the nucleus via a Pomeron, }\DIFdelend %DIF > In diffractive photoproduction, the momentum-transfer t distribution is known to reflect the transverse spatial structure of the interaction. In particular, a steeper t dependence is generally associated with larger effective transverse configurations~\cite{Kuroda:2017ogq,Kowalski:2006hc,Nemchik:1996cw}. In this context, comparing the t spectra of the resonant and non-resonant $\pi^+\pi^-$ contributions provides a way to probe potential differences in their underlying transverse dipole size.
\DIFaddbegin \DIFadd{In diffractive photoproduction, the momentum-transfer $|t|$ distribution primarily reflects the transverse spatial profile of the target through its form factor. At the same time, it can also be sensitive to }\DIFaddend the \DIFdelbegin \DIFdel{Drell-S${\rm \ddot{o}ding}$ process serves as a sensitive probe of the nuclear gluon structure, the nuclear saturation and shadowing effect in $\pi^+/\pi^-$-p diffraction scattering~\mbox{%DIFAUXCMD
\cite{ZEUS:1997rof,Laget:2019tou}}\hspace{0pt}%DIFAUXCMD
.
%DIF < In addition, the 
}%DIFDELCMD < 

%DIFDELCMD < %%%
%DIF < Recently, as  it was realized that the Drell-S${\rm \ddot{o}ding}$ process
%DIF < Hereinafter, the Drell-S${\rm \ddot{o}ding}$ process was introduced to modify the $\rho^0$ mass shape in phenomenological models and measurements.%in most of measurements of the exclusive $\pi^+\pi^-$ production in
%DIF < Due to the specific one-pion-exchange mechanism and the smallness of the $\pi$ mass, the Drell-S${\rm \ddot{o}ding}$ process is expected to be softer than $\rho^0$ photoproduction and can be correlated to hadron-induced processes~\cite{pumplin1970diffraction}.
\DIFdelend \DIFaddbegin \DIFadd{transverse size of the interacting dipole via the convolution of the photon and hadronic wavefunctions with the scattering amplitude. In particular, a steeper $|t|$ dependence is generally associated with larger effective transverse configurations~\mbox{%DIFAUXCMD
\cite{Kuroda:2017ogq,Kowalski:2006hc,Nemchik:1996cw}}\hspace{0pt}%DIFAUXCMD
.
In this context, comparing the $|t|$ spectra of the resonant and non-resonant $\pi^+\pi^-$ contributions within the same mass and rapidity range provides a way to probe potential differences in their underlying transverse dipole sizes.
%DIF > Compared to the resonance $\rho^0$, the direct $\pi^+\pi^-$ is more loosely bound with a larger dipole size and corresponding to a smaller pair $p_T$, as implied by the transverse size–momentum uncertainty relation.
%DIF > It is dominated by the virtual $\pi$–nucleus scattering diagrams~\cite{pumplin1970diffraction,bolz2015photoproduction}, for both $\pi^+/$–nucleus and $\pi^-$–nucleus scattering as depicted in Fig.~\ref{fig:1}.
}\DIFaddend 

Vector meson photoproduction, e.g., $\rho^0$ and $J/\psi$, has been measured extensively in ultraperipheral collisions (UPCs) of heavy ions~\cite{alice2021coherent,acharya2019coherent,STAR:2017enh,abelev2008rho,STAR:2019yox,STAR:2002caw,afanasiev2009photoproduction,guzey2013evidence,ALICE:2020ugp,ALICE:2024ife,collaboration2021first,GlueX:2024erj,Pybus:2024ifi,GlueX:2019mkq}. 
However, the non-resonant \DIFdelbegin \DIFdel{Drell-Söding }\DIFdelend \DIFaddbegin \DIFadd{Drell-S${\rm \ddot{o}ding}$ }\DIFaddend process remains poorly characterized due to its small cross section and overlap with resonant $\rho^0$.
%DIF > The Drell-S${\rm \ddot{o}ding}$ term cannot be isolated event-by-event and is extracted through its interference with the $\rho^0$ photoproduction.
\DIFaddbegin \DIFadd{The Drell-S${\rm \ddot{o}ding}$ term cannot be isolated on an event-by-event basis and is extracted statistically after subtracting known contributions, relying on its interference with the $\rho^0$ photoproduction.
}\DIFaddend In previous $\rho^0$ measurements, the Drell-S${\rm \ddot{o}ding}$ component is treated with an unknown amplitude formulated as a constant~\cite{STAR:2017enh,abelev2008rho,STAR:2019yox,STAR:2002caw,ALICE:2020ugp} or a parameterised function~\cite{H1:2020lzc,ZEUS:2011tzw}. 
\DIFdelbegin \DIFdel{However, when isolating the }\DIFdelend %DIF > However, when isolating the Drell-S${\rm \ddot{o}ding}$ contribution, replacing the constant approximation with a model-calculated spectrum results in a deviation over $15\%$ of the extracted Drell-S${\rm \ddot{o}ding}$ cross section. 
\DIFaddbegin \DIFadd{The extracted }\DIFaddend Drell-S${\rm \ddot{o}ding}$ contribution \DIFdelbegin \DIFdel{, replacing the constant approximation with a model-calculated spectrum results in a deviation over $15\%$ of the extracted Drell-S${\rm \ddot{o}ding}$ cross section}\DIFdelend \DIFaddbegin \DIFadd{depends on the assumed mass dependence of this term}\DIFaddend . Therefore, adopting a more realistic spectrum derived from model calculations \DIFdelbegin \DIFdel{is crucial to achieve }\DIFdelend \DIFaddbegin \DIFadd{would be desirable to achieve a more }\DIFaddend precise measurements of the Drell-S${\rm \ddot{o}ding}$ process.
%DIF > Experimentally, the Drell-S${\rm \ddot{o}ding}$ contribution cannot be isolated event-by-event; instead, it is extracted through its interference with the $\rho^0$ amplitude that shapes the exclusive $\pi^+\pi^-$ mass spectrum.
With growing interest in exclusive hadronic pair production~\cite{sciadv.abq3903,Brandenburg:2024ksp,TOTEM:2024aso,ALICE:2023kgv,STAR:2020dzd,ATLAS:2022uef}, precise measurements of the Drell-S${\rm \ddot{o}ding}$ process offer a new handle to quantify decay-induced effects in nuclear tomography and \DIFdelbegin \DIFdel{entanglement enabled spin-interference (EESI ) }\DIFdelend \DIFaddbegin \DIFadd{EESI }\DIFaddend via comparisons with $\rho^0$ photoproduction. A precise characterization of the Drell-S${\rm \ddot{o}ding}$ process is also \DIFdelbegin \DIFdel{essential }\DIFdelend \DIFaddbegin \DIFadd{important }\DIFaddend for disentangling excited $\rho^0$ states, e.g., $\rho(1450)$ and $\rho(1700)$, in exclusive $\pi^+\pi^-$ production~\cite{ALICE:2020ugp}.
%The Drell-S${\rm \ddot{o}ding}$ process could provide a novel probe to the nuclear gluon densities
%provides a unique opportunity to study the photon hadronic $\pi^+\pi^-$ and $\rho^0$ structure by comparison to $\rho^0$ photoproduction and the gluonic structure of nucleus.
%The variation for the Drell-S${\rm \ddot{o}ding}$ mass shape implemented has a negligible impact on the obtained $\rho^0$ cross section but leads to an obvious uncertainty ($\sim15\%$) for the Drell-S${\rm \ddot{o}ding}$. It is one of the most pressing tasks to apply a more real form for precise measurement of the Drell-S${\rm \ddot{o}ding}$ process in high energy nuclear UPC physics.

% main content of the measurement
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend In this Letter, we report a comprehensive analysis for a series of simultaneous measurements of exclusive $\pi^{+}\pi^{-}$ production. For the first time, (\romannumeral1) the $|t|$ dependence of the Drell-S${\rm \ddot{o}ding}$ process cross section is precisely measured; (\romannumeral2) EESI for the Drell-S${\rm \ddot{o}ding}$ process is measured through ${\rm A_{2\Delta\phi}}$; \DIFaddbegin \DIFadd{and }\DIFaddend (\romannumeral3) \DIFdelbegin \DIFdel{We measure how }\DIFdelend \DIFaddbegin \DIFadd{the dependence of }\DIFaddend ${\rm A_{2\Delta\phi}}$ \DIFaddbegin \DIFadd{on the pair invariant mass is measured }\DIFaddend for exclusive $\pi^+\pi^-$ pair production\DIFdelbegin \DIFdel{depends on pair invariant mass related to the incident photon energy. The }\DIFdelend \DIFaddbegin \DIFadd{. Finally, the }\DIFaddend ${\rm A_{2\Delta\phi}}$ data are compared with vector meson dominant (VMD)~\cite{PhysRevD.103.033007,Zha:2018jin} and non-resonance production (NRP) calculations~\DIFdelbegin \DIFdel{\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,Zha:2018jin}}\hspace{0pt}%DIFAUXCMD
}\DIFdelend \DIFaddbegin \DIFadd{\mbox{%DIFAUXCMD
\cite{pumplin1970diffraction,Zha:2018jin,Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend .

\DIFdelbegin %DIFDELCMD < \begin{figure}[h]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.45\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{Figure1 pancake nucleus.png}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{Schematic view of the production mechanism for Drell-S${\rm \ddot{o}ding}$ process. A virtual photon fluctuates into an entangled $\pi^{+}\pi^{-}$ pair during the strong interaction time ($\sim 2\times10^{-24}$s). One single virtual $\pi^{+}/\pi^{-}$ is diffraction-scattered on the nucleus. The wavy structures represent local energy fluctuations in the strong electromagnetic field, while the associated blue and red balls depict short-lived pair fluctuations due to the local energy excitations. }
%DIFDELCMD <   \label{fig:1}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\DIFdelend %DIF >  \begin{figure}[h]
%DIF >    \centering
%DIF >    \begin{minipage}{0.45\textwidth}
%DIF >      \includegraphics[width=\textwidth]{Figure1 pancake nucleus.png}
%DIF >    \end{minipage}
%DIF >    \caption{A schematic diagram showing the production of entangled pions via the Drell-S${\rm \ddot{o}ding}$ process. A virtual photon fluctuates into an entangled $\pi^{+}\pi^{-}$ pair during the strong interaction time and one of the pions is diffraction-scattered off the nucleus. The wavy structures in the background represent local energy fluctuations in the strong electromagnetic field, while the associated blue and red balls depict short-lived pair fluctuations due to the local energy excitations. }
%DIF >    \label{fig:1}
%DIF >  \end{figure}
\DIFaddbegin \begin{figure}[t]
\centering

\begin{minipage}{0.325\columnwidth}
\centering
\includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_1_largetext.eps}\hfill
%\\ (\romannumeral1)
\end{minipage}
\begin{minipage}{0.325\columnwidth}
\centering
\includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_2_largetext.eps}\hfill
%\\ (\romannumeral2)
\end{minipage}
%\vspace{0.2cm}
\begin{minipage}{0.325\columnwidth}
\centering
\includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_3_largetext.eps}
% \\ (\romannumeral3)
\end{minipage}
% \begin{minipage}{0.47\columnwidth}
% \centering
% \includegraphics[width=\linewidth]{GPCreviewfigure/feynman_diag_4.eps}
% \\ (\romannumeral4)
% \end{minipage}
\caption{Diagrams of Drell-S${\rm \ddot{o}ding}$ $\pi^{+}\pi^{-}$ production: (left and middle) dominant diagrams corresponding to $\pi^+-$nucleus and $\pi^--$nucleus scattering; (right) $\pi^+\pi^--$nucleus coupling diagram}
\label{fig:1}
\end{figure}
\DIFaddend %The wavy structures represent local energy fluctuations, while the blue and red virtual particle pairs depict short-lived quantum vacuum fluctuations in the electromagnetic field.

% Data detector and trigger

The measurement of exclusive $\pi^{+}\pi^{-}$ production \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend conducted in Au+Au UPCs at $\sqrt{s_{NN}}=200$ GeV at the Relativistic Heavy Ion Collider (RHIC) using the Solenoidal Tracker at RHIC (STAR)~\cite{STAR:detector}. An inclusive UPC trigger \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend applied for the pre-selection to the data~\cite{star:trigger}. This \DIFdelbegin \DIFdel{UPC trigger relies }\DIFdelend \DIFaddbegin \DIFadd{trigger relied }\DIFaddend on rapidity gaps defined by the small beam-beam counter (BBC) tiles on both sides \DIFaddbegin \DIFadd{of the detector }\DIFaddend ($3<\eta<5$)~\cite{star-bbc1,star:bbc2}, low activity in the mid-rapidity in the barrel time-of-flight (TOF) system~\cite{star:tof,Chen:2024aom} (TOF multiplicity between 1 and 7), and the coincidence of neutrons hitting both the east and west zero degree calorimeters (ZDC)~\cite{star:zdc,Xu:2016alq}. \DIFdelbegin \DIFdel{We analyze a total of 135 million triggered events collected in 2010, 2011, and 2014. }\DIFdelend The integrated luminosities for the triggered \DIFdelbegin \DIFdel{datasets }\DIFdelend \DIFaddbegin \DIFadd{data sets }\DIFaddend recorded in 2010, 2011, and 2014 are 679\DIFdelbegin \DIFdel{$\pm$ 68}\DIFdelend , 859\DIFdelbegin \DIFdel{$\pm$ 86}\DIFdelend , and 1464 \DIFdelbegin \DIFdel{$\pm$ 146 }\DIFdelend $\mu b^{-1}$ \DIFaddbegin \DIFadd{with 10\% uncertainty}\DIFaddend , respectively. The momenta of charged-particle tracks \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend reconstructed by the time projection chamber (TPC) covering pseudorapidities $\vert \eta \vert<1.0$ for the full azimuthal angle ($0<\phi<2\pi$)~\cite{star:tpc}. %The TPC also provides the specific ionization loss (dE/dx) measurement for the particle identification of each tracks.
The TPC also \DIFdelbegin \DIFdel{provides }\DIFdelend \DIFaddbegin \DIFadd{provided }\DIFaddend specific ionization energy loss (dE/dx) measurements for particle identification, which \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend used to construct the deviation parameter $n\sigma_\pi$ by comparing the measured dE/dx to the value predicted for a pion.


Further offline \DIFdelbegin \DIFdel{selections are }\DIFdelend \DIFaddbegin \DIFadd{cuts on the events were }\DIFaddend required. Events \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend required to have a primary vertex reconstructed by a pair of charged-particle tracks with a longitudinal distance of $\vert V_z \vert<100$ cm to the nominal center of STAR. The associated charged-particle tracks \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend required to have at least 15 fit points and 10 dE/dx points to ensure sufficient momentum and dE/dx resolutions. Charged-particle tracks \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend required to match to TOF hits \DIFaddbegin \DIFadd{in order }\DIFaddend to mitigate the effect of out-of-time pileup. The distance of closest approach (DCA) for charged-particle tracks \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend required to be less than 1.5 cm to the primary collision vertex to suppress contamination by secondary decay particles. High purity $\pi^{+}\pi^{-}$ pairs \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend selected by requiring $\chi^2_{\pi\pi}=n\sigma_{\pi 1}^2+n\sigma_{\pi 2}^2<8$, which \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend almost fully efficient ($\sim99\%$). 
\DIFdelbegin \DIFdel{The azimuthal decay }\DIFdelend %DIF > The azimuthal decay angle $\Delta\phi$ is calculated as $\Delta\phi = \phi_{\pi} - \phi_{\text{pair}}$, where $\phi_{\pi}$ is the azimuthal angle of the $\pi^+$ or $\pi^-$ in the $\pi^+\pi^-$ rest frame and $\phi_{\text{pair}}$ is the azimuthal angle of the pair momentum in the laboratory frame. 
\DIFaddbegin \DIFadd{The azimuthal }\DIFaddend angle $\Delta\phi$ is \DIFdelbegin \DIFdel{calculated as $\Delta\phi = \phi_{\pi} - \phi_{\text{pair}}$, where $\phi_{\pi}$ is the azimuthal angle }\DIFdelend \DIFaddbegin \DIFadd{defined in the transverse plane as the angle between $\vec{p}_{T1}+\vec{p}_{T2}$ and $\vec{p}_{T1}-\vec{p}_{T2}$, where $\vec{p}_{T1}$ and $\vec{p}_{T2}$ are the transverse momenta }\DIFaddend of the
$\pi^+$ \DIFdelbegin \DIFdel{or }\DIFdelend \DIFaddbegin \DIFadd{and }\DIFaddend $\pi^-$\DIFdelbegin \DIFdel{in the $\pi^+\pi^-$ rest frame and $\phi_{\text{pair}}$ is the azimuthal angle of the pair momentum in the laboratory frame}\DIFdelend .
Over one million exclusive $\pi^{+}\pi^{-}$ pairs \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend selected in the invariant mass region $0.6<M_{\pi^+\pi^-}<0.9$ GeV/${\rm c^2}$, enabling precise differential spectra studies.

% embedding and efficiency correction
A Monte Carlo (MC) sample \DIFdelbegin \DIFdel{is generatedwith $V_z$ distributions }\DIFdelend \DIFaddbegin \DIFadd{of photoproduced $\pi^+\pi^-$ pairs was generated. The kinematic distributions were weighted according to the model described in Ref.~\mbox{%DIFAUXCMD
\cite{Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
. The vertex ($V_z$) distribution was }\DIFaddend matched to data. The sample \DIFdelbegin \DIFdel{passes }\DIFdelend \DIFaddbegin \DIFadd{data was passed }\DIFaddend through the STAR detector response \DIFdelbegin \DIFdel{simulation based on }\DIFdelend \DIFaddbegin \DIFadd{simulator using }\DIFaddend GEANT3~\cite{Brun:1119728} to evaluate the acceptance and detector efficiency. It \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend then embedded into randomly recorded STAR events that \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend tuned to reproduce the ZDC \DIFdelbegin \DIFdel{confidence }\DIFdelend \DIFaddbegin \DIFadd{coincidence }\DIFaddend rate during data taking, ensuring realistic background effects on charged-particle track and vertex reconstruction. To \DIFdelbegin \DIFdel{reduce the model dependence}\DIFdelend \DIFaddbegin \DIFadd{minimize potential biases arising from the Monte Carlo sample's underlying kinematic distributions}\DIFaddend , a high-dimensional correction \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend employed to obtain the cross section as
\begin{equation}
    \frac{d^3 \sigma}{d p_T d M d \Delta \phi} =\frac{N\left(p_T, M, \Delta \phi\right)}{\varepsilon_{\text {trig }}{\text{corr}}(p_T, M, \Delta \phi)L\Delta p_T\Delta M\Delta(\Delta \phi)},
\end{equation}
where $\varepsilon_{\text {trig }}$ is the trigger efficiency; $\text{corr}(p_T, M, \Delta \phi)$ represents the $p_T$, $M$, and $\Delta \phi$-dependent acceptance and efficiency correction; and $L$ is the integrated luminosity. Since signals \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend corrected with the $\Delta \phi$ dependence, the amplitudes of the $\Delta \phi$ modulations at all orders \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend corrected simultaneously. In addition, the momentum smearing of charged-particle tracks in \DIFaddbegin \DIFadd{the }\DIFaddend TPC smooths the $\Delta \phi$ spectra, especially at low $\pi^{+}\pi^{-}$ $p_T$. We \DIFdelbegin \DIFdel{estimate }\DIFdelend \DIFaddbegin \DIFadd{estimated }\DIFaddend the momentum resolution impact and unfold the measured ${\rm A_{2\Delta\phi}}$ based on the ratio of the reconstructed ${\rm A_{2\Delta\phi}}$ to the original in the polarized Monte Carlo simulation\DIFaddbegin \DIFadd{, where the $\Delta\phi$ distribution was reweighted according to the polarization model}\DIFaddend .
% different processes separation (mass fitting)

\DIFdelbegin \begin{displaymath}
\DIFdel{\begin{aligned}
\frac{d \sigma}{d M_{\pi^{+} \pi^{-}}} &= \left| A_\rho \frac{\sqrt{M_{\pi \pi} M_{\rho} \Gamma_\rho}}{M_{\pi \pi}^2-M_\rho^2+i M_\rho \Gamma_\rho} f_{fluxcorr} + B f_{S\ddot{o}ding} \right. \\ 
&\left. + C_\omega e^{i \phi_\omega} \frac{\sqrt{M_{\pi \pi} M_\omega \Gamma_{\omega \rightarrow \pi \pi}}}{M_{\pi \pi}^2-M_\omega^2+i M_\omega \Gamma_\omega} \right|^2 + f_{\mu\mu} + f_{\text {bg}}.
\end{aligned}
%DIFDELCMD < \label{eq:fit}%%%
}\end{displaymath}%DIFAUXCMD
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend An improved description of the exclusive $\pi^{+}\pi^{-}$ mass distribution \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend constructed to separate the resonance and non-resonance components from different processes, as expressed in Eq.~\ref{eq:fit}. In this parameterization, $A_\rho$ and $C_\omega$ denote the amplitudes for $\rho^0$ and $\omega$, respectively; $B$ represents the magnitude of the normalized model-calculated Drell-S${\rm \ddot{o}ding}$ mass shape $f_{S\ddot{o}ding}$; \DIFdelbegin \DIFdel{and }\DIFdelend $\phi_\omega$ is the mixing phase angle for $\omega$\DIFaddbegin \DIFadd{; and $f_{\text {bg}}$ is a linear polynomial that accounts for any residual non-photoproduction background}\DIFaddend . We apply the relativistic Breit-Wigner (rBW) resonance for $\rho^0$ and $\omega$, and a phenomenological non-resonance by the NRP calculation\DIFaddbegin \DIFadd{~\mbox{%DIFAUXCMD
\cite{Wu:2026emu}}\hspace{0pt}%DIFAUXCMD
}\DIFaddend . The momentum-dependent mass widths are expressed as~\cite{Alvensleben:1971hz}
% Fitting mass figure
\begin{equation}
\begin{aligned}
&\Gamma_\rho=\Gamma_0 \frac{M_\rho}{M_{\pi \pi}}\left(\frac{M_{\pi \pi}^2-4 m_\pi^2}{M_\rho^2-4 m_\pi^2}\right)^{3 / 2},\\
&\Gamma_{\omega \rightarrow \pi \pi}=\operatorname{Br}(\omega \rightarrow \pi \pi) \Gamma_0 \frac{M_\omega}{M_{\pi \pi}}\left(\frac{M_{\pi \pi}^2-4 m_\pi^2}{M_\omega^2-4 m_\pi^2}\right)^{3 / 2},
\end{aligned}
\end{equation}
with $\operatorname{Br}(\omega \rightarrow \pi \pi)=0.0153^{+0.0011}_{-0.0013}$~\cite{ParticleDataGroup:2014cgo}, where $\Gamma_0$ is the pole \DIFdelbegin \DIFdel{meson width }\DIFdelend \DIFaddbegin \DIFadd{width for each meson}\DIFaddend . 
The vector meson photoproduction amplitude \DIFdelbegin \DIFdel{could be }\DIFdelend \DIFaddbegin \DIFadd{is }\DIFaddend modeled as the photon energy distribution and scattering amplitude for the virtual vector meson and nucleus. Due to the correlation of the photon energy and vector meson mass, $E_{\gamma}=M/2\times exp(\pm y)$, the photon energy distribution \DIFdelbegin \DIFdel{would }\DIFdelend slightly modify the rBW mass spectra. This correction, $f_{fluxcorr}$, is considered using VMD model calculation~\cite{PhysRevD.103.033007,Zha:2018jin}. The $\gamma\gamma \rightarrow \mu^+ \mu^-$ process constitutes a \DIFdelbegin \DIFdel{non-negligible }\DIFdelend background, as muons cannot be distinguished from pions due to the absence of a start time $t_0$ measurement for TOF. Dimuon production, $f_{\mu\mu}$, is calculated using lowest-order QED~\cite{Li:2023yjt,Zha:2018tlq,Zha:2021jhf}, which \DIFdelbegin \DIFdel{has been demonstrated to describe the experimental measurement well}\DIFdelend \DIFaddbegin \DIFadd{reproduces experimental data}\DIFaddend ~\cite{STAR:2018ldd,STAR:2019wlg}.


\DIFaddbegin \begin{equation}
\DIFadd{\begin{aligned}
\frac{d \sigma}{d M_{\pi^{+} \pi^{-}}} &= \left| A_\rho \frac{\sqrt{M_{\pi \pi} M_{\rho} \Gamma_\rho}}{M_{\pi \pi}^2-M_\rho^2+i M_\rho \Gamma_\rho} f_{fluxcorr} + B f_{S\ddot{o}ding} \right. \\ 
&\left. + C_\omega e^{i \phi_\omega} \frac{\sqrt{M_{\pi \pi} M_\omega \Gamma_{\omega \rightarrow \pi \pi}}}{M_{\pi \pi}^2-M_\omega^2+i M_\omega \Gamma_\omega} \right|^2 + f_{\mu\mu} + f_{\text {bg}}.
\end{aligned}
\label{eq:fit}
}\end{equation}
\DIFaddend %Where $A_\rho$ and $C_\omega$ are the amplitudes for $\rho^0$ and $\omega$, respectively. The $\phi_\omega$ is the mixing phase angle for $\omega$. The momentum-dependent mass widths are expressed as~\cite{Alvensleben:1971hz}
% Fitting mass figure


\DIFdelbegin %DIFDELCMD < \begin{figure}[h]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.495\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{mass_fit_tot_run10_0.6_1.3_11_10_25.eps}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{The differential cross section $d^2\sigma/dM_{\pi\pi}dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $p_T<0.1$ GeV/c and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV, together with illustration of the fitting algorithm to separate resonance and continuum components. The black markers show the data, and the lilac markers show the Drell-S${\rm \ddot{o}ding}$ term. The interference terms for $\rho$-Söding (purple), $\omega$-Söding (brown), and $\rho-\omega$ (dark green) are shown. $\mu^+\mu^-$ pair production is represented by the blue band.}
%DIFDELCMD <   \label{fig:2}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \begin{figure}[h]
  \centering
  \begin{minipage}{0.495\textwidth}
    \includegraphics[width=\textwidth]{GPCreviewfigure/mass_fit_tot_run10_0.6_1.3_4_6_26.eps}
  \end{minipage}
   \caption{The differential cross section $d^2\sigma/dM_{\pi\pi}dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $p_T<0.1$ GeV/c and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV, together with an illustration of the fitting algorithm to separate the $\rho^{0}$ and Drell-S${\rm \ddot{o}ding}$ components. The black markers show the data, and the lilac line show the Drell-S${\rm \ddot{o}ding}$ term. The interference terms for $\rho$-Söding (purple), $\omega$-Söding (brown), and $\rho-\omega$ (dark green) are shown. $\mu^+\mu^-$ pair production is represented by the blue band.}
  \label{fig:2}
\end{figure}
\DIFaddend 


\DIFdelbegin %DIFDELCMD < \begin{figure}[h]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.48\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{GPCreviewfigure/paper_dt_ratio_theocomp_mass0609.eps}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{(top) The differential cross section $d\sigma/d|t|dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $0.6<M<0.9$ GeV/${\rm c^2}$ and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. The blue and red markers (lines) represent the measured (calculated) $\rho^0$ photoproduction~\cite{Zha:2018jin} and Drell-S${\rm \ddot{o}ding}$ process~\cite{pumplin1970diffraction,bolz2015photoproduction}, respectively. (bottom) The measured (calculated) ratio of the Drell-S${\rm \ddot{o}ding}$ to $\rho^0$ photoproduction cross sections provides insight into the photon’s hadronic structure and indicates a softer production mechanism.}
%DIFDELCMD <   \label{fig:3}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \begin{figure}[h]
  \centering
  \begin{minipage}{0.48\textwidth}
    \includegraphics[width=\textwidth]{GPCreviewfigure/paper_dt_ratio_theocomp_mass0609.eps}
  \end{minipage}
   \caption{(top) The differential cross section $d^{2}\sigma/d|t|dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $0.6<M<0.9$ GeV/${\rm c^2}$ and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. The blue and red markers (lines) represent the measured (calculated) $\rho^0$ photoproduction~\cite{Zha:2018jin} and Drell-S${\rm \ddot{o}ding}$ process~\cite{pumplin1970diffraction,bolz2015photoproduction,Wu:2026emu}, respectively. EPA denotes the equivalent photon approximation. (bottom) The measured (calculated) ratio of the Drell-S${\rm \ddot{o}ding}$ to $\rho^0$ photoproduction cross sections.} 
   %provides insight into the photon’s hadronic structure and indicates a softer production mechanism.}
  \label{fig:3}
\end{figure}
\DIFaddend %The theoretical calculation, however, does not reproduce the measured trend.
%DIF < The Drell-S${\rm \ddot{o}ding}$ term is represented by a normalized model-calculated mass shape $f_{S\ddot{o}ding}$, scaled by a free parameter $B$ that reflects its magnitude. 
%DIF < Correction for the rBW $\rho^0$ induced by the photon energy distribution is considered by the VMD model calculation as $f_{fluxcorr}$~\cite{PhysRevD.103.033007,Zha:2018jin}. The vector meson photoproduction amplitude could be modeled as the photon energy distribution and scattering amplitude for the virtual vector meson and nucleus. Due to the correlation of the photon energy and vector meson mass, $E_{\gamma}=M/2\times exp(\pm y)$, the photon energy distribution would slightly modify the rBW mass spectra. Dimuon production is calculated using lowest-order QED~\cite{Li:2023yjt,Zha:2018tlq,Zha:2021jhf}, incorporating both parallel and cross diagrams, which has been demonstrated to describe the experimental measurement well~\cite{STAR:2018ldd,STAR:2019wlg}.

\DIFdelbegin %DIFDELCMD < \begin{figure*}[ht]
%DIFDELCMD <   \centering
%DIFDELCMD <   \begin{minipage}{0.96\textwidth}
%DIFDELCMD <     \includegraphics[width=\textwidth]{paper_a2_pt_mass_11_7_25.eps}
%DIFDELCMD <   \end{minipage}
%DIFDELCMD <    \caption{The second order modulation amplitude $A_{2\Delta\phi}$ as functions of the pair transverse momentum $p_T$ (left) and the invariant mass $M_{\pi^+\pi^-}$ (right) for $0<p_T<0.1$ GeV/c, $0.6<M_{\pi^+\pi^-}<0.9$ GeV/${\rm c^2}$, and $\vert y \vert<0.9$ in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV. The Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction are shown in red and teal points. Statistic uncertainties and systematic uncertainties are represented by the error bars and boxes (left), or band (right) respectively. The model calculations are donated as dash lines.}
%DIFDELCMD <   \label{fig:4}
%DIFDELCMD < \end{figure*}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin \begin{figure*}[ht]
  \centering
  \begin{minipage}{0.96\textwidth}
    \includegraphics[width=\textwidth]{GPCreviewfigure/paper_a2_pt_mass_4_2_26.eps}
  \end{minipage}
   \caption{The $\Delta\phi$ distributions normalized to unit integral (left); second-order modulation amplitude $A_{2\Delta\phi}$ versus pair transverse momentum $p_T$ (middle) and invariant mass $M_{\pi^+\pi^-}$ (right) in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV. The Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction data points are shown as red and teal points. Statistical uncertainties and systematic uncertainties are represented by the error bars and boxes (middle), or bands (left and right) respectively. The model calculations are denoted as dashed lines. In the middle panel, the data and model calculations use the same binning in $p_T$. For clarity, the $\rho^0$ and Drell–S${\rm \ddot{o}ding}$ data points are slightly shifted horizontally relative to the bin centers to avoid overlap.}
  \label{fig:4}
\end{figure*}
\DIFaddend 

%DIF > The correlated uncertainties are estimated to be 2% and 5% of the extracted yields for $\rho^0$ and Drell-Söding
%Systematic uncertainty
Systematic uncertainties are classified into correlated and uncorrelated components \DIFaddbegin \DIFadd{among different data sets}\DIFaddend . Correlated uncertainties \DIFdelbegin \DIFdel{, }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend estimated to be 2\% for $\rho^0$ and 5\% for Drell-Söding, \DIFdelbegin \DIFdel{arise }\DIFdelend \DIFaddbegin \DIFadd{arising }\DIFaddend mainly from the fitting procedure, including \DIFdelbegin \DIFdel{the choice }\DIFdelend \DIFaddbegin \DIFadd{choices }\DIFaddend of fitting range and the modeling of the Drell-S${\rm \ddot{o}ding}$ mass shape. The \DIFdelbegin \DIFdel{fitting stability is }\DIFdelend \DIFaddbegin \DIFadd{fitting-range dependence was }\DIFaddend evaluated by varying the \DIFdelbegin \DIFdel{lower }\DIFdelend \DIFaddbegin \DIFadd{low }\DIFaddend mass boundary from 0.6 GeV/${\rm c^2}$ to 0.57 GeV/${\rm c^2}$ and 0.65 GeV/${\rm c^2}$.
An alternative parametrization of the non-resonant amplitude, $A_{nr}= f_{nr}/(m_{\pi\pi}^2-4m_\pi^2+\Lambda_{nr}^2)^{\delta_{nr}}$, following Ref.~\cite{H1:2020lzc}, \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend used to assess the model dependence \DIFdelbegin \DIFdel{. }\DIFdelend \DIFaddbegin \DIFadd{of the fit to the data, }\DIFaddend where $f_{n r}$, $\Lambda_{n r}$, and $\delta_{n r}$ are free parameters. 
%While this approach enhances model flexibility, it introduces sensitivity to local minima during the fitting process.
Uncorrelated uncertainties \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend evaluated through variations in topological selection criteria and adjustments to the MC model in acceptance and efficiency extractions. Uncorrelated uncertainties are about 5\% for $\rho^0$ photoproduction and 8\% for Drell-S${\rm \ddot{o}ding}$. An external 10\% uncertainty in integrated luminosity determination and a 3\% per-track reconstruction uncertainty \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend included. 
Results from different \DIFdelbegin \DIFdel{datasets }\DIFdelend \DIFaddbegin \DIFadd{data sets }\DIFaddend are statistically consistent within uncertainties and are combined using a weighted average based on the quadratic sum of statistical and uncorrelated systematic uncertainties. The \DIFaddbegin \DIFadd{statistical and uncorrelated systematic uncertainties were treated as independent and were propagated to the combined result by summing their contributions in quadrature with the corresponding weights.
The correlated systematic uncertainties, assumed to be fully correlated across data sets, were combined by taking their weighted average.
The correlations between $\rho^0$ photoproduction and Drell-S${\rm \ddot{o}ding}$ were accounted for through the covariance matrix in the fit.
The }\DIFaddend total systematic uncertainty \DIFdelbegin \DIFdel{is obtained by combining }\DIFdelend \DIFaddbegin \DIFadd{was obtained by adding }\DIFaddend the uncorrelated and correlated uncertainties in quadrature. 
%DIF < The results of each dataset are consistent within uncertainties and combined with the weight using the statistic uncertainties and uncorrelated systematic uncertainties.
\DIFaddbegin \DIFadd{The systematic uncertainty sources and evaluation procedure are the same for the extracted $A_{2\Delta\phi}$. For the difference between the $A_{2\Delta\phi}$ of $\rho^0$ and Drell-S${\rm \ddot{o}ding}$, the uncertainty was evaluated directly on the difference, such that the correlations between them are naturally included.
%DIF > The results of each data set are consistent within uncertainties and combined with the weight using the statistic uncertainties and uncorrelated systematic uncertainties.
}\DIFaddend %\begin{equation}
%    \begin{aligned}
        %&w_i = \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}/W,\\ \text{where} \ &W=\sum_i \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}.
%        w_i = \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}/(\sum_i \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}).
%    \end{aligned}
%\end{equation}
%The total systematic uncertainty is obtained by combining the uncorrelated and correlated uncertainties in quadrature.


Figure~\ref{fig:2} illustrates the differential cross section $d^2\sigma/dM_{\pi\pi}dy$ as a function of the invariant mass $M_{\pi\pi}$.
%in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. 
The data points represent the measured cross section, while the red curve shows the full fit incorporating various contributing components.
%DIF < The dominant $\rho^0$ rBW accounts for the primary resonance structure, with additional contributions from the $\omega$ rBW component and the Drell-Söding process. The interference terms, including $\rho$-Söding, $\omega$-Söding, and $\omega$-$\rho$ interference, modulate the overall shape. The shaded blue region represents the background from $\gamma\gamma \rightarrow \mu^+\mu^-$ process. The enhancement of the cross section of $\gamma\gamma \rightarrow \mu^+\mu^-$ by setting the $\mu$ tracks with the $\pi$ mass is considered in QED calculations.
%DIF < addsomething here 1 DS is a small contribution however we could still precise measure it due to the key role for the interference in determining the cross section 
Although the Drell-S${\rm \ddot{o}ding}$ process constitutes a relatively minor contribution to exclusive $\pi^+\pi^-$ production, its interference with the $\rho^0$ production crucially shapes the observed mass spectrum. The mass shift and the asymmetric structure of the mass peak are both governed by this interference thus enabling a precise extraction of the Drell-Söding contribution. \DIFdelbegin \DIFdel{We perform mass fits per pair }\DIFdelend \DIFaddbegin \DIFadd{Mass spectra were fitted independently in each (}\DIFaddend $p_T$\DIFdelbegin \DIFdel{and }\DIFdelend \DIFaddbegin \DIFadd{, }\DIFaddend $\Delta \phi$\DIFdelbegin \DIFdel{to disentangle the differential cross section for each process.
}\DIFdelend \DIFaddbegin \DIFadd{) bin to extract the contributions of the different processes and evaluate the corresponding cross sections.
%DIF > We perform mass fits per pair $p_T$ and $\Delta \phi$ to disentangle the differential cross section for each process.
}\DIFaddend %Although the Drell-S${\rm \ddot{o}ding}$ process accounts for a relatively small contribution of the exclusive $\pi^+\pi^-$ production, the interference of the Drell-S${\rm \ddot{o}ding}$ and $\rho^0$ production plays a key role in shaping the mass spectrum. 
%DIF < The fact that the mass shift and the shape of both sides of the mass peak are determined by the interference effect between the Drell-S${\rm \ddot{o}ding}$ and $\rho^0$ production ensures the feasibility of precisely measuring the Drell-Söding process. We perform mass fits per pair $p_T$ and $\Delta \phi$ to measure the differential cross section for each process. 
Amplitudes of the second order cosine modulation ${\rm A_{2\Delta\phi}}$ \DIFdelbegin \DIFdel{could be }\DIFdelend \DIFaddbegin \DIFadd{was }\DIFaddend reconstructed by a weighted sum ${\rm A_{2\Delta\phi}}=\sum_{i=1}^n 2N_i{\rm cos(2\Delta \phi_i)}$, %DIF > where $N_i$ is the normalized yield at $\Delta \phi_i$. 
where $N_i$ \DIFdelbegin \DIFdel{is the normalized yield at }\DIFdelend \DIFaddbegin \DIFadd{denotes the yield in each }\DIFaddend $\Delta \phi_i$ \DIFdelbegin \DIFdel{. 
%DIF < The quality of the fits is quantified by the reduced chi-square, $\chi^2/\text{ndf}$, which ranges from 50 to 100 per 65 degrees of freedom ($50/65\sim100/65$) for mass fits performed in different $p_T$, $\Delta\phi$ and $p_T-\Delta\phi$ bins.
}\DIFdelend \DIFaddbegin \DIFadd{bin normalized by the total yield in the corresponding $p_T$ interval.
}\DIFaddend The fit quality is \DIFdelbegin \DIFdel{evaluated }\DIFdelend \DIFaddbegin \DIFadd{quantified }\DIFaddend using the reduced chi-square ($\chi^2/\text{ndf}$), which ranges from 50 to 100 per 65 degrees of freedom, reflecting consistent modeling of the spectral features.

%DIF < Fig.~\ref{fig:3} shows the differential cross section $d^2\sigma/dp_T^2dy$ for Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction with their ratio on the pair $p_T$ dependence. The Drell-S${\rm \ddot{o}ding}$ exhibit a sharper decreasing slope with $p_T$ increase and an obviously smaller $p_T$ for the diffractive dips which are related to the nucleus imaging. The ratio shows a significant bump which definitively demonstrate Drell-S${\rm \ddot{o}ding}$ process is softer than the $\rho^0$ production although they are both $\gamma A \rightarrow \pi^+\pi^-A$ processes. The results indicate the photon hadronic structure that the virtual $\pi^+\pi^-$ pair fluctuation concentrate more at lower photon energy region compared to virtual $\rho^0$.
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend % gpt improved:
Figure~\ref{fig:3} presents the differential cross-section $d^2\sigma/d|t| dy$ for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction, along with their ratio as a function of \DIFdelbegin \DIFdel{$|t|$}\DIFdelend \DIFaddbegin \DIFadd{$|t| \approx p_{T\pi^{+}\pi^{-}}^{2}$}\DIFaddend . The $\rho^0$ results are consistent with the previous measurement~\cite{STAR:2017enh}.
%DIF < The Drell-S${\rm \ddot{o}ding}$ process exhibits a steeper decline with increasing $p_T$ compared to $\rho^0$ photoproduction, with a noticeably lower $p_T$ position for the diffractive minima, which are associated with nuclear imaging. 
Compared to $\rho^0$ photoproduction, the Drell-S${\rm \ddot{o}ding}$ process exhibits a steeper decline with increasing $|t|$ with its diffractive minima shifted to lower $|t|$, reflecting a softer production mechanism and differences in the underlying photon hadronic structure.
The measured ratio reveals a pronounced bump at low $|t|$, suggesting that the virtual $\pi^+\pi^-$ configuration is spatially broader than the $\rho^0$ state. Theoretical calculations do not reproduce this trend, possibly due to missing dipole-size effects that are not accounted for in the model.

Figure~\ref{fig:4} shows the azimuthal anisotropy \DIFaddbegin \DIFadd{(left)}\DIFaddend , quantified by the second-order cosine modulation amplitude, ${\rm A_{2\Delta\phi}}$, for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction as functions of the pair transverse momentum $p_T$ (\DIFdelbegin \DIFdel{left}\DIFdelend \DIFaddbegin \DIFadd{middle}\DIFaddend ) and the invariant mass $M_{\pi^+\pi^-}$ (right) within rapidity $|y|<0.9$. 
The amplitudes \DIFdelbegin \DIFdel{, }\DIFdelend ${\rm A_{2\Delta\phi}}$ \DIFdelbegin \DIFdel{, are determined by performing invariant mass fits }\DIFdelend \DIFaddbegin \DIFadd{were then extracted from the fitted yields }\DIFaddend in distinct $\Delta\phi$ or $p_T$\DIFdelbegin \DIFdel{-vs-}\DIFdelend \DIFaddbegin \DIFadd{--}\DIFaddend $\Delta\phi$ intervals.
To ensure sufficient statistical precision for resolving subtle features in the mass distribution, the $p_T$ range is divided into three bins: $0 < p_T < 0.03~\mathrm{GeV}/c$, $0.03 < p_T < 0.05~\mathrm{GeV}/c$, and $0.05 < p_T < 0.1~\mathrm{GeV}/c$. The resulting \DIFdelbegin \DIFdel{differential cross section as a function of }\DIFdelend $\Delta\phi$ \DIFdelbegin \DIFdel{is }\DIFdelend \DIFaddbegin \DIFadd{distributions are }\DIFaddend then used to extract the $\cos(2\Delta\phi)$ modulation amplitude. 
%DIF < Fig.~\ref{fig:4} presents the azimuthal anisotropy quantified by the amplitude of the second order cosine modulation $A_{2\Delta\phi}$ for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction as functions of the pair transverse momentum $p_T$ (left) and the invariant mass $M_{\pi^+\pi^-}$ (right) for rapidity $|y|<0.9$. In order to measure the amplitudes $A_{2\Delta\phi}$, the mass fits are performed in different $\Delta\phi$ or $p_T-\Delta\phi$ intervals. The pair $p_T$ is divided into three bins as $0<p_T<0.03$ GeV/c, $0.03<p_T<0.05$ GeV/c and $0.05<p_T<0.1$ GeV/c for the differential mass fits in $p_T-\Delta\phi$ intervals. This is to guarantee enough statistics for a series of good fits to the subtle mass shape. Consequently, the obtained differential cross section as a function of $\Delta\phi$ is used to reconstruct the amplitude of $cos(2(\Delta\phi))$ modulation. The mass dependence of the amplitude $A_{2\Delta\phi}$ in an integrated pair transverse momentum $0<p_T<0.1$ GeV/c is presented in the right figure.
The ${\rm A_{2\Delta\phi}}$ of the Drell-S${\rm \ddot{o}ding}$ process exhibits a similar $p_T$ dependence \DIFdelbegin \DIFdel{with the }\DIFdelend \DIFaddbegin \DIFadd{as }\DIFaddend $\rho^0$ photoproduction and \DIFaddbegin \DIFadd{has }\DIFaddend an enhancement in transverse momentum in the range $0.05<p_T<0.1$ GeV/c. 
%DIF < For exclusive $\pi^+\pi^-$ production, the yield in this $p_T$ intervals constitutes about half of the yield over $0<p_T<0.1$ GeV/c. The Drell-S${\rm \ddot{o}ding}$ is known to have a softer $p_T$ distribution compared to $\rho^0$ from Fig.~\ref{fig:3}. 
The right panel illustrates the $M_{\pi^+\pi^-}$ dependence of ${\rm A_{2\Delta\phi}}$\DIFdelbegin \DIFdel{integrated over the full $p_T$ range, $0 < p_T < 0.1~\mathrm{GeV}/c$. 
The $A_{2\Delta\phi}$ is found to have a relatively flat }\DIFdelend \DIFaddbegin \DIFadd{. 
%DIF > integrated over the full $p_T$ range, $0 < p_T < 0.1~\mathrm{GeV}/c$. 
%DIF > The ${\rm A_{2\Delta\phi}}$ is found to have a relatively flat $M_{\pi^+\pi^-}$ dependence
No significant }\DIFaddend $M_{\pi^+\pi^-}$ dependence \DIFdelbegin \DIFdel{, suggesting minimal }\DIFdelend \DIFaddbegin \DIFadd{of ${\rm A_{2\Delta\phi}}$ is found, indicating no strong }\DIFaddend photon energy dependence in EESI. Notably, the \DIFdelbegin \DIFdel{measured }\DIFdelend \DIFaddbegin \DIFadd{extracted }\DIFaddend ${\rm A_{2\Delta\phi}}$ for the Drell-S${\rm \ddot{o}ding}$ \DIFaddbegin \DIFadd{process }\DIFaddend is systematically higher than that for $\rho^0$ photoproduction.
\DIFdelbegin \DIFdel{When integrated over }\DIFdelend \DIFaddbegin \DIFadd{For $0 < p_T < 0.1~\mathrm{GeV}/c$, $|y| < 0.9$, and }\DIFaddend $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$, \DIFdelbegin \DIFdel{the difference corresponds to a significance of 4.6~$\sigma$, evaluated including all statistical and systematic uncertainties. Specifically, }\DIFdelend \DIFaddbegin \DIFadd{the extracted }\DIFaddend ${\rm A_{2\Delta\phi}}$ values \DIFdelbegin \DIFdel{for $0 < p_T < 0.1~\mathrm{GeV}/c$, $|y| < 0.9$ and $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$ are measured as $0.2702 \pm 0.0024 \pm 0.0120$ }\DIFdelend \DIFaddbegin \DIFadd{are $0.273 \pm 0.010 \pm 0.013$ }\DIFaddend (Drell-S${\rm \ddot{o}ding}$) and \DIFdelbegin \DIFdel{$0.2181 \pm 0.0022 \pm 0.0050$ }\DIFdelend \DIFaddbegin \DIFadd{$0.219 \pm 0.003 \pm 0.005$ }\DIFaddend ($\rho^0$ photoproduction). The first quoted errors are statistical uncertainties\DIFaddbegin \DIFadd{, }\DIFaddend while the second are \DIFdelbegin \DIFdel{systematical uncertainties. %DIF < Notably, the measured ${\rm A_{2\Delta\phi}}$ as a function of $M_{\pi^+\pi^-}$ for the Drell-S${\rm \ddot{o}ding}$ in $0 < p_T < 0.1~\mathrm{GeV}/c$ is systematically higher than that for $\rho^0$ photoproduction. When integrated over $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$, the difference corresponds to a significance of $4.6\sigma$, evaluated including all statistical and systematic uncertainties. Specifically, ${\rm A_{2\Delta\phi}}$ values for $0 < p_T < 0.1~\mathrm{GeV}/c$, $|y| < 0.9$ and $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$ are measured as $0.2702 \pm 0.0024 \pm 0.0120$ (Drell-S${\rm \ddot{o}ding}$) and $0.2181 \pm 0.0022 \pm 0.0050$ ($\rho^0$ photoproduction). The first quoted errors are statistical uncertainties while the second are systematical uncertainties.
}\DIFdelend \DIFaddbegin \DIFadd{systematic uncertainties. The resulting difference is $0.054 \pm 0.010 \pm 0.015$, corresponds to a significance of 3.0~$\sigma$ when statistical and systematic uncertainties are included. 
}\DIFaddend 

The predictions of the EPA-VMD and NRP model are also compared with the data and found to \DIFdelbegin \DIFdel{understimate }\DIFdelend \DIFaddbegin \DIFadd{underestimate }\DIFaddend $A_{2\Delta\phi}$ at \DIFdelbegin \DIFdel{lower }\DIFdelend \DIFaddbegin \DIFadd{low }\DIFaddend transverse momentum, $0<p_T<0.05$ GeV/c. 
\DIFdelbegin \DIFdel{Based on the $A_{2\Delta\phi}$ measurement, specific contributions to the difference for the exclusive resonance and non-resonance produced entangled $\pi^+\pi^-$ pairs in cooperation with EESI can be studied. }\DIFdelend The results show no \DIFdelbegin \DIFdel{clear coherence lost in scattering with a nucleusand no clear destructive interference caused by the }\DIFdelend \DIFaddbegin \DIFadd{evidence, within the present uncertainties, for a loss of coherence in scattering off a nucleus, nor for destructive interference induced by the difference between the }\DIFaddend $\pi^+p$ and $\pi^-p$ scattering \DIFdelbegin \DIFdel{asymmetric }\DIFdelend amplitudes in the Drell-S${\rm \ddot{o}ding}$ process.
%DIF < It is also indicated no significant wave function collapse caused by the $\rho^0$ decay


% Final conclusion generated by DS
In conclusion, we report the observation of EESI in the Drell-S${\rm \ddot{o}ding}$ process and the pair $p_T$ and $M$ dependence of the differential cross section for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV at RHIC. A model-based Drell-S${\rm \ddot{o}ding}$ shape is employed to separate different processes involved in exclusive $\pi^+\pi^-$ production. 
%DIF < The Drell-S${\rm \ddot{o}ding}$ process is observed obviously softer from the pair $p_T$ spectrum compared to $\rho^0$ photoproduction. 
The observation of EESI effects demonstrates that the non-resonant $\pi^+\pi^-$ pairs are entangled in the Drell-S${\rm \ddot{o}ding}$ process. The amplitude, ${\rm A_{2\Delta\phi}}$, for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction are found to have similar decreasing trends along the pair $p_T$. Compared to \DIFaddbegin \DIFadd{the }\DIFaddend $\rho^0$, an enhancement is observed \DIFdelbegin \DIFdel{for }\DIFdelend \DIFaddbegin \DIFadd{in }\DIFaddend the Drell-S${\rm \ddot{o}ding}$ process \DIFdelbegin \DIFdel{for }\DIFdelend \DIFaddbegin \DIFadd{in }\DIFaddend pair $p_T$ in the range $0.05<p_T<0.1$ GeV/c. The measured ${\rm A_{2\Delta\phi}}$ for these processes is found to have no obvious pair mass $M_{\pi^+\pi^-}$ dependence, and the amplitude ${\rm A_{2\Delta\phi}}$ for Drell-S${\rm \ddot{o}ding}$ is \DIFdelbegin \DIFdel{4.6 }\DIFdelend \DIFaddbegin \DIFadd{3.0 }\DIFaddend $\sigma$ higher than for $\rho^0$ photoproduction \DIFdelbegin \DIFdel{among }\DIFdelend \DIFaddbegin \DIFadd{over }\DIFaddend the observed mass regions. Moreover, the observed Drell-S${\rm \ddot{o}ding}$ $|t|$ spectrum is softer when compared to $\rho^0$ photoproduction. \DIFdelbegin \DIFdel{A comprehensive analysis of the measurements is reported through the comparison between resonant and non-resonant $\pi^+\pi^-$ photoproduction. }\DIFdelend These results advance the exploration of quantum interference phenomena in photon–nucleus interactions, providing a basis for future investigations in ultraperipheral heavy-ion collisions.%DIF > A comprehensive analysis of the measurements is reported through the comparison between resonant and non-resonant $\pi^+\pi^-$ photoproduction. These results advance the exploration of quantum interference phenomena in photon–nucleus interactions, providing a basis for future investigations in ultraperipheral heavy-ion collisions.

%The exclusive $\pi^+\pi^-$ production can be measured as a probe to the nuclear gluon density and nuclear geometry. From the comparison between the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction, the photon hadronic structure by fluctuation to ($\rho^0$ and $\pi^+\pi^-$) and production mechanism could be studied with its impact on imaging the nucleus. 
%Acknowledgement
\DIFdelbegin \section*{\DIFdel{Acknowledgement}}
%DIFAUXCMD
\DIFdelend \DIFaddbegin 

\textit{\DIFadd{Acknowledgments}}\DIFadd{—}\DIFaddend We thank the RHIC Operations Group and SDCC at BNL, the NERSC Center at LBNL, and the Open Science Grid consortium for providing resources and support.  This work was supported in part by the Office of Nuclear Physics within the U.S. DOE Office of Science, the U.S. National Science Foundation, National Natural Science Foundation of China, Chinese Academy of Science, the Ministry of Science and Technology of China and the Chinese Ministry of Education, NSTC Taipei, the National Research Foundation of Korea, Czech Science Foundation and Ministry of Education, Youth and Sports of the Czech Republic, Hungarian National Research, Development and Innovation Office, New National Excellency Programme of the Hungarian Ministry of Human Capacities, Department of Atomic Energy and Department of Science and Technology of the Government of India, the National Science Centre and WUT ID-UB of Poland, German Bundesministerium f\"ur Bildung, Wissenschaft, Forschung and Technologie (BMBF), Helmholtz Association, Ministry of Education, Culture, Sports, Science, and Technology (MEXT), and Japan Society for the Promotion of Science (JSPS).
\DIFdelbegin %DIFDELCMD < \bibliography{reference}
%DIFDELCMD < %%%
\DIFdelend \DIFaddbegin 

\bibliography{referencenew}
\DIFaddend 











==> test.tex <==
%\label{sec:dataselection}

% physics：
% 1. mass ordering image the nucleus
% %%%% nuclear force (need pi N cross section)
% 2. novel probe for deep understanding the interference
% 3. comparason to rho:    
% how does different photon hadronic structure
% production mechanics
% affect imagining the nucleus and the interference


% Introduction:
% nuclear and vacuum structure
% photoproduction used for parton dis both sides
% Entanglement interference
% unsolved issue & It is of great interest to investigate...
% In this Letter, we present
% The data and the trigger
% Event track pid cut and observable recon
% 

%The vacuum under the extremely strong electromagnetic field produced in relativistic heavy ion collisions has a subtle partonic structure. The photon induced processes, vector meson photoproduction and photon photon process, have been extensively measured

%The extremely strong electromagnetic field generated in the relativistic heavy-ion collisions can be described as a co-moving photon cloud with beams~\cite{weizsacker1934ausstrahlung,williams1934nature}, and thus enables photon nuclear interactions~\cite{krauss1997photon}. In the scenario of such interactions, a photon fluctuates into a virtual vector meson or hadron-antihadron pair, which then scatters off the nucleus by Pomeron exchange (finite sum of gluon ladders). Therefore, photon-nuclear interactions provide a unique probe of the photon's hadronic structure~\cite{bauer1978hadronic,AbdulKhalek:2021gbh,Li:2022kwn} and serve as a complementary tool for studying key nuclear properties, including the nuclear gluon distributions~\cite{guzey2013exclusive} and the overall nuclear size~\cite{sciadv.abq3903,Klein:1999qj}.
Ultra-strong electromagnetic fields in relativistic heavy-ion collisions manifest as a comoving photon cloud accompanying the nuclei~\cite{weizsacker1934ausstrahlung,williams1934nature}, enabling photonuclear interactions. In these processes, a photon fluctuates into a virtual vector meson or hadron-antihadron pair, which scatters via Pomeron exchange (gluonic exchanges). Such interactions provide a unique probe of the photon's hadronic structure~\cite{bauer1978hadronic,AbdulKhalek:2021gbh,Li:2022kwn} and serve as a complementary tool for studying key nuclear properties, including nuclear gluon distributions~\cite{guzey2013exclusive} and the overall nuclear size~\cite{sciadv.abq3903,Klein:1999qj}.


For a quasi-real photon with spin-1, dissociation processes must adhere to angular momentum conservation. The photon may fluctuate into either (\romannumeral1) a virtual vector meson, which retains the photon’s spin and parity quantum numbers $(J^{PC}=1^{--})$, or (\romannumeral2) a virtual hadron-antihadron pair, giving rise to non-resonant photoproduction, known as the Drell-S${\rm \ddot{o}ding}$ process. Since both nuclei can act as photon emitters or targets, the emission source (nucleus A or B) becomes almost indistinguishable, establishing a ``double-slit'' interference pattern at the femtometer scale~\cite{sciadv.abq3903,PhysRevD.103.033007}. This interference induces second-order cosine oscillations in the asymmetries of the decay angular $\Delta\phi$ distributions~\cite{xing2020cos}. In the Drell-S${\rm \ddot{o}ding}$ mechanism, the relativistic $\pi^{+}\pi^{-}$ pair emerges via photon-nuclear interaction and rapidly separates in nearly opposite directions. %at relativistic speeds. 
The pair resembles an Einstein-Podolsky-Rosen (EPR) system~\cite{Brandenburg:2024ksp} with no further information transmission after production. %Due to limited overlap between the outgoing pion wave packets~\cite{klein2000interference}, the interference pattern may be partially suppressed. 
It is of great interest to investigate in depth the interference and entanglement in the Drell-S${\rm \ddot{o}ding}$ process. 

%It is a chance to explore the effect of decay in comparison to the production with an intermediate state such as $\rho^0$. 


The Drell-S${\rm \ddot{o}ding}$ process has two dominant diagrams through virtual $\pi^+/\pi^-$-nucleus scattering depicted in Fig~\ref{fig:1}. And another for the gauge invariance~\cite{pumplin1970diffraction,bolz2015photoproduction}. In 1960, Drell first proposed the diagrams of this process as promising contributions to secondary beams via the $\gamma \rightarrow \pi^+\pi^-$ process at SLAC~\cite{drell1960production}. Later in 1966, S${\rm \ddot{o}ding}$ calculated them to explain the observed skewing of the $\rho^0$ resonance peak~\cite{soding1966apparent}. Compared to the resonance $\rho^0$, the direct $\pi^+\pi^-$ is more loosely bounded with a larger dipole size, corresponding to a smaller pair $p_T$ even at the same photon energy. With such a system scattering from the nucleus via a Pomeron, the Drell-S${\rm \ddot{o}ding}$ process serves as a sensitive probe of the nuclear gluon structure, the nuclear saturation and shadowing effect in $\pi^+/\pi^-$-p diffraction scattering~\cite{ZEUS:1997rof,Laget:2019tou}. %In addition, the 

%Recently, as  it was realized that the Drell-S${\rm \ddot{o}ding}$ process
%Hereinafter, the Drell-S${\rm \ddot{o}ding}$ process was introduced to modify the $\rho^0$ mass shape in phenomenological models and measurements.%in most of measurements of the exclusive $\pi^+\pi^-$ production in
%Due to the specific one-pion-exchange mechanism and the smallness of the $\pi$ mass, the Drell-S${\rm \ddot{o}ding}$ process is expected to be softer than $\rho^0$ photoproduction and can be correlated to hadron-induced processes~\cite{pumplin1970diffraction}.


Vector meson photoproduction, e.g., $\rho^0$ and $J/\psi$, has been measured extensively in ultraperipheral collisions (UPCs) of heavy ions~\cite{alice2021coherent,acharya2019coherent,STAR:2017enh,abelev2008rho,STAR:2019yox,STAR:2002caw,afanasiev2009photoproduction,guzey2013evidence,ALICE:2020ugp,ALICE:2024ife}. %However, due to the difficulties to isolate the small nonresonance contribution in exclusive $\pi^+\pi^-$ production, the Drell-S${\rm \ddot{o}ding}$ process has hardly been precisely measured and mostly introduced for $\rho^0$ analysis to explain the skewed mass shape. 
However, the non-resonant Drell-Söding process---a subdominant contribution to exclusive $\pi^+\pi^-$ production---remains poorly characterized due to its small cross section and overlap with resonant $\rho^0$.
In previous measurements, the Drell-S${\rm \ddot{o}ding}$ component is treated with an unknown amplitude formulated as a constant~\cite{STAR:2017enh,abelev2008rho,STAR:2019yox,STAR:2002caw,ALICE:2020ugp} or a parameterised function~\cite{H1:2020lzc,ZEUS:2011tzw}. For $\rho^0$ measurements, a crude description of the Drell-S${\rm \ddot{o}ding}$ process remains sufficient, as its contribution is relatively small and does not significantly impact the overall measurement. However, when isolating the Drell-S${\rm \ddot{o}ding}$ contribution, replacing the constant approximation with a model-calculated spectrum results in a deviation over $15\%$ of the extracted Drell-S${\rm \ddot{o}ding}$ cross section. Therefore, adopting a more realistic spectrum derived from model calculations is crucial to achieve precise measurements of the Drell-S${\rm \ddot{o}ding}$ process. 

Recently, with increasing interest in exclusive hadronic pair production~\cite{sciadv.abq3903,Brandenburg:2024ksp,TOTEM:2024aso,ALICE:2023kgv,STAR:2020dzd,ATLAS:2022uef}, it has been realized that precise measurements of the Drell-S${\rm \ddot{o}ding}$ process could provide a new avenue to investigate the interplay of the decay process, production mechanisms in nuclear tomography, and spin-interference effect through comparisons with $\rho^0$ photoproduction. Furthermore, a precise characterization of the Drell-S${\rm \ddot{o}ding}$ process is of paramount importance for disentangling excited $\rho^0$ states, e.g., $\rho(1450)$ and $\rho(1700)$) in exclusive $\pi^+\pi^-$ production~\cite{ALICE:2020ugp}.
%The Drell-S${\rm \ddot{o}ding}$ process could provide a novel probe to the nuclear gluon densities
%provides a unique opportunity to study the photon hadronic $\pi^+\pi^-$ and $\rho^0$ structure by comparison to $\rho^0$ photoproduction and the gluonic structure of nucleus.
%The variation for the Drell-S${\rm \ddot{o}ding}$ mass shape implemented has a negligible impact on the obtained $\rho^0$ cross section but leads to an obvious uncertainty ($\sim15\%$) for the Drell-S${\rm \ddot{o}ding}$. It is one of the most pressing tasks to apply a more real form for precise measurement of the Drell-S${\rm \ddot{o}ding}$ process in high energy nuclear UPC physics.

% main content of the measurement

In this Letter, we report a comprehensive analysis for a series of simultaneous measurements of exclusive $\pi^{+}\pi^{-}$ production. For the first time, (\romannumeral1) the $p_T$ dependence of the Drell-S${\rm \ddot{o}ding}$ process cross section is precisely measured; (\romannumeral2) spin-interference for the Drell-S${\rm \ddot{o}ding}$ process is measured through ${\rm A_{2\Delta\phi}}$; (\romannumeral3) We measure how ${\rm A_{2\Delta\phi}}$ for exclusive $\pi^+\pi^-$ pair production depends on pair invariant mass related to the incident photon energy. The ${\rm A_{2\Delta\phi}}$ data are compared with vector meson dominant (VMD)~\cite{PhysRevD.103.033007,Zha:2018jin} and non-resonance production (NRP) calculations~\cite{pumplin1970diffraction,Zha:2018jin}.

\begin{figure}[h]
  \centering
  \begin{minipage}{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figure1 pancake nucleus.png}
  \end{minipage}
   \caption{Schematic view of the production mechanism for Drell-S${\rm \ddot{o}ding}$ process. A virtual photon fluctuates into an entangled $\pi^{+}\pi^{-}$ pair during the strong interaction time ($\sim 2\times10^{-24}$s). One single virtual $\pi^{+}/\pi^{-}$ is diffraction-scattered on the nucleus. The wavy structures represent local energy fluctuation in the strong electromagnetic field, while the associated blue and red balls depict short-lived pair fluctuation due to the local energy excitations. }
  \label{fig:1}
\end{figure}
%The wavy structures represent local energy fluctuations, while the blue and red virtual particle pairs depict short-lived quantum vacuum fluctuations in the electromagnetic field.

% Data detector and trigger

The measurement of exclusive $\pi^{+}\pi^{-}$ production is conducted in Au+Au UPCs at $\sqrt{s_{NN}}=200$ GeV at the Relativistic Heavy Ion Collider (RHIC) using the Solenoidal Tracker at RHIC (STAR)~\cite{STAR:detector}. An inclusive UPC trigger is applied for the pre-selection to the data~\cite{star:trigger}. This UPC trigger relies on rapidity gaps defined by the small beam-beam counter (BBC) tiles on both sides ($3<\eta<5$)~\cite{star-bbc1,star:bbc2}, low activity in the mid-rapidity in the barrel time-of-flight (TOF) system~\cite{star:tof} (TOF multiplicity between 1 and 7), and the coincidence of neutrons hitting both east and west zero degree calorimeters (ZDC)~\cite{star:zdc}. We analyze a total of 135 million triggered events collected in 2010, 2011, and 2014. The integrated luminosities for the triggered datasets recorded in 2010, 2011, and 2014 are 679$\pm$68, 859$\pm$86, and 1464$\pm$146 $\mu b^{-1}$, respectively. The momenta of charged-particle tracks are reconstructed by the time projection chamber (TPC) covering pseudorapidities $\vert \eta \vert<1.0$ for the full azimuthal angle ($0<\phi<2\pi$)~\cite{star:tpc}. %The TPC also provides the specific ionization loss (dE/dx) measurement for the particle identification of each tracks.
The TPC also provides specific ionization energy loss (dE/dx) measurements for particle identification, which are used to construct the deviation parameter $n\sigma_\pi$ by comparing the measured dE/dx to the value predicted for a pion.

We analyze a total of 135 million triggered events collected in 2010, 2011, and 2014.
To select UPC events that might contain exclusive $\pi^{+}\pi^{-}$ pairs, further offline selections are required. We require a primary vertex reconstructed by a pair of charged-particle tracks with a longitudinal distance of $\vert V_z \vert<100$ cm to the nominal center of STAR. The associated charged-particle tracks are required to have at least 15 fit points and 10 dE/dx points to ensure sufficient momentum and dE/dx resolutions. Charged-particle tracks are required to match to TOF hits to mitigate the effect of out-of-time pileup. The distance of closest approach (DCA) for charged-particle tracks is required to be less than 1.5 cm to the primary collision vertex to suppress contamination by secondary decay particles. High purity $\pi^{+}\pi^{-}$ pairs are selected by requiring $\chi^2_{\pi\pi}=n\sigma_{\pi 1}^2+n\sigma_{\pi 2}^2<8$, which is almost fully efficient ($\sim99\%$). The azimuthal decay angle $\Delta\phi$ is calculated as $\Delta\phi = \phi_{\pi} - \phi_{\text{pair}}$, where $\phi_{\pi}$ is the azimuthal angle of the $\pi^+$ or $\pi^-$ in the $\pi^+\pi^-$ rest frame and $\phi_{\text{pair}}$ is the azimuthal angle of the pair momentum in the laboratory frame. In total, over one million exclusive $\pi^{+}\pi^{-}$ pairs are reconstructed in the invariant mass region $0.6<M_{\pi^+\pi^-}<0.9$ GeV/${\rm c^2}$, enabling precise differential spectra studies.
%guaranteeing good statistics for differential spectra studies.

% embedding and efficiency correction

A Monte Carlo (MC) sample was generated with kinematic distributions weighted according to model calculations~\cite{PhysRevD.103.033007,Zha:2018jin} and $V_z$ distributions matched to data. The sample passes through the STAR detector response simulation based on GEANT3~\cite{Brun:1119728} to evaluate the acceptance and detector efficiency. This sample is embedded into randomly recorded STAR events that are tuned to reproduce the ZDC confidence rate during data taking, ensuring realistic background effects on charged-particle track and vertex reconstruction. To reduce the model dependence, a high-dimensional correction is employed to obtain the cross section as
\begin{equation}
    \frac{d^3 \sigma}{d p_T d M d \Delta \phi} =\frac{N\left(p_T, M, \Delta \phi\right)}{\varepsilon_{\text {trig }}{\text{corr}}(p_T, M, \Delta \phi)L\Delta p_T\Delta M\Delta(\Delta \phi)},
\end{equation}
where $\varepsilon_{\text {trig }}$ is the trigger efficiency; $\text{corr}(p_T, M, \Delta \phi)$ represents the $p_T$, $M$, and $\Delta \phi$-dependent acceptance and efficiency correction; and $L$ is the integrated luminosity. Since signals are corrected with the $\Delta \phi$ dependence, the amplitudes of the $\Delta \phi$ modulations at all orders are corrected simultaneously. In addition, the momentum smearing of charged-particle tracks in TPC smooths the $\Delta \phi$ spectra, especially at low $\pi^{+}\pi^{-}$ $p_T$. We estimate the momentum resolution impact and unfold the measured ${\rm A_{2\Delta\phi}}$ based on the ratio of the reconstructed ${\rm A_{2\Delta\phi}}$ to the original in the polarized Monte Carlo simulation.


\begin{figure}[h]
  \centering
  \begin{minipage}{0.495\textwidth}
    \includegraphics[width=\textwidth]{mass_fit_tot_run10_0.6_1.3_11_10_25.eps}
  \end{minipage}
   \caption{The differential cross section $d^2\sigma/dM_{\pi\pi}dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $p_T<0.1$ GeV/c and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV, together with illustration of the fitting algorithm to separate resonance and continuum components. The black markers show the data, and the lilac markers show the Drell-S${\rm \ddot{o}ding}$ term. The interference terms for $\rho$-Söding (purple), $\omega$-Söding (brown), and $\rho-\omega$ (dark green) are shown. $\mu^+\mu^-$ pair production is represented by the blue band.}
  \label{fig:2}
\end{figure}



% different processes separation (mass fitting)
An improved description of the exclusive $\pi^{+}\pi^{-}$ mass distribution is constructed to separate the resonance and non-resonance components from different processes. We apply the relativistic Breit-Wigner (rBW) resonance for $\rho^0$ and $\omega$, and a phenomenological non-resonance by the NRP calculation. The $\gamma\gamma \rightarrow \mu^+ \mu^-$ process constitutes a significant background, as muons cannot be distinguished from pions due to the absence of a start time $t_0$ measurement for TOF. The separation of those components is achieved by simultaneous mass fits, formulated as

\begin{equation}
\begin{aligned}
\frac{d \sigma}{d M_{\pi^{+} \pi^{-}}} &= \left| A_\rho \frac{\sqrt{M_{\pi \pi} M_{\rho} \Gamma_\rho}}{M_{\pi \pi}^2-M_\rho^2+i M_\rho \Gamma_\rho} f_{fluxcorr} + B f_{S\ddot{o}ding} \right. \\ 
&\left. + C_\omega e^{i \phi_\omega} \frac{\sqrt{M_{\pi \pi} M_\omega \Gamma_{\omega \rightarrow \pi \pi}}}{M_{\pi \pi}^2-M_\omega^2+i M_\omega \Gamma_\omega} \right|^2 + f_{\mu\mu} + f_{\text {bg}}.
\end{aligned}
\end{equation}
Where $A_\rho$ and $C_\omega$ are the amplitudes for $\rho^0$ and $\omega$, respectively. The $\phi_\omega$ is the mixing phase angle for $\omega$. The momentum-dependent mass widths are expressed as~\cite{Alvensleben:1971hz}
% Fitting mass figure



\begin{equation}
\begin{aligned}
&\Gamma_\rho=\Gamma_0 \frac{M_\rho}{M_{\pi \pi}}\left(\frac{M_{\pi \pi}^2-4 m_\pi^2}{M_\rho^2-4 m_\pi^2}\right)^{3 / 2},\\
&\Gamma_{\omega \rightarrow \pi \pi}=\operatorname{Br}(\omega \rightarrow \pi \pi) \Gamma_0 \frac{M_\omega}{M_{\pi \pi}}\left(\frac{M_{\pi \pi}^2-4 m_\pi^2}{M_\omega^2-4 m_\pi^2}\right)^{3 / 2},
\end{aligned}
\end{equation}
with $\operatorname{Br}(\omega \rightarrow \pi \pi)=0.0153^{+0.0011}_{-0.0013}$~\cite{ParticleDataGroup:2014cgo}, where $\Gamma_0$ is the pole meson width.
\begin{figure}[h]
  \centering
  \begin{minipage}{0.48\textwidth}
    \includegraphics[width=\textwidth]{GPCreviewfigure/paper_dt_ratio_theocomp_mass0609.eps}
  \end{minipage}
   \caption{(top) The differential cross section $d\sigma/d|t|dy$ of exclusive $\pi^{+}\pi^{-}$ production for pair $0.6<M<0.9$ GeV/${\rm c^2}$ and $|y|<0.9$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. The blue and red markers (lines) represent the measured (calculated) $\rho^0$ photoproduction~\cite{Zha:2018jin} and Drell-S${\rm \ddot{o}ding}$ process~\cite{pumplin1970diffraction,bolz2015photoproduction}, respectively. (bottom) The measured (calculated) ratio of the Drell-S${\rm \ddot{o}ding}$ to $\rho^0$ photoproduction cross sections provides insight into the photon’s hadronic structure and indicates a softer production mechanism. The theoretical calculation, however, does not reproduce the measured trend.}
  \label{fig:3}
\end{figure}
The Drell-S${\rm \ddot{o}ding}$ term is represented by a normalized model-calculated mass shape $f_{S\ddot{o}ding}$, scaled by a free parameter $B$ that reflects its magnitude. 
Correction for the rBW $\rho^0$ induced by the photon energy distribution is considered by the VMD model calculation as $f_{fluxcorr}$~\cite{PhysRevD.103.033007,Zha:2018jin}. The vector meson photoproduction amplitude could be modeled as the photon energy distribution and scattering amplitude for the virtual vector meson and nucleus. Due to the correlation of the photon energy and vector meson mass, $E_{\gamma}=M/2\times exp(\pm y)$, the photon energy distribution would slightly modify the rBW mass spectra. Dimuon production is calculated using lowest-order QED~\cite{Li:2023yjt,Zha:2018tlq,Zha:2021jhf}, incorporating both parallel and cross diagrams, which has been demonstrated to describe the experimental measurement well~\cite{STAR:2018ldd,STAR:2019wlg}.

\begin{figure*}[ht]
  \centering
  \begin{minipage}{0.96\textwidth}
    \includegraphics[width=\textwidth]{paper_a2_pt_mass_11_7_25.eps}
  \end{minipage}
   \caption{The second order modulation amplitude $A_{2\Delta\phi}$ as functions of the pair transverse momentum $p_T$ (left) and the invariant mass $M_{\pi^+\pi^-}$ (right) for $0<p_T<0.1$ GeV/c, $0.6<M_{\pi^+\pi^-}<0.9$ GeV/${\rm c^2}$, and $\vert y \vert<0.9$ in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV. The Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction are shown in red and teal points. Statistic uncertainties and systematic uncertainties are represented by the error bars and boxes (left), or band (right) respectively. The model calculations are donated as dash lines.}
  \label{fig:4}
\end{figure*}

Figure~\ref{fig:2} illustrates the differential cross section $d^2\sigma/dM_{\pi\pi}dy$ as a function of the invariant mass $M_{\pi\pi}$ in Au+Au UPCs at $\sqrt{s_{NN}} = 200$~GeV. The data points represent the measured cross section, while the red curve shows the full fit incorporating various contributing components. The dominant $\rho^0$ rBW accounts for the primary resonance structure, with additional contributions from the $\omega$ rBW component and the Drell-Söding process. The interference terms, including $\rho$-Söding, $\omega$-Söding, and $\omega$-$\rho$ interference, modulate the overall shape. The shaded blue region represents the background from $\gamma\gamma \rightarrow \mu^+\mu^-$ process. The enhancement of the cross section of $\gamma\gamma \rightarrow \mu^+\mu^-$ by setting the $\mu$ tracks with the $\pi$ mass is considered in QED calculations.

%addsomething here 1 DS is a small contribution however we could still precise measure it due to the key role for the interference in determining the cross section 
%Although the Drell-S${\rm \ddot{o}ding}$ process accounts for a relatively small contribution of the exclusive $\pi^+\pi^-$ production, the interference of the Drell-S${\rm \ddot{o}ding}$ and $\rho^0$ production plays a key role in shaping the mass spectrum. 
Although the Drell-S${\rm \ddot{o}ding}$ process constitutes a relatively minor contribution to exclusive $\pi^+\pi^-$ production, its interference with the $\rho^0$ production crucially shapes the observed mass spectrum. The mass shift and the asymmetric structure of the mass peak are both governed by this interference thus enabling a precise extraction of the Drell-Söding contribution.  We perform mass fits per pair $p_T$ and $\Delta \phi$ to disentangle the differential cross section for each process.
%The fact that the mass shift and the shape of both sides of the mass peak are determined by the interference effect between the Drell-S${\rm \ddot{o}ding}$ and $\rho^0$ production ensures the feasibility of precisely measuring the Drell-Söding process. We perform mass fits per pair $p_T$ and $\Delta \phi$ to measure the differential cross section for each process. 
Amplitudes of the second order cosine modulation ${\rm A_{2\Delta\phi}}$ could be reconstructed by a weighted sum ${\rm A_{2\Delta\phi}}=\sum_{i=1}^n 2N_icos(\Delta \phi_i)$, where $N_i$ is the normalized yield at $\Delta \phi_i$. 
%The quality of the fits is quantified by the reduced chi-square, $\chi^2/\text{ndf}$, which ranges from 50 to 100 per 65 degrees of freedom ($50/65\sim100/65$) for mass fits performed in different $p_T$, $\Delta\phi$ and $p_T-\Delta\phi$ bins.
The fit quality is evaluated using the reduced chi-square ($\chi^2/\text{ndf}$), which ranges from 50 to 100 per 65 degrees of freedom ($50/65\sim100/65$) across $p_T$, $\Delta\phi$, reflecting consistent modeling of the spectral features.


%Systematic uncertainty
Systematic uncertainties are evaluated in two categories: correlated and uncorrelated uncertainties. Correlated uncertainties are estimated at approximately 2\% for $\rho^0$ photoproduction and 5\% for Drell-S${\rm \ddot{o}ding}$ process, mainly due to the fitting range and ambiguities in modeling the Drell-S${\rm \ddot{o}ding}$ mass shape. To evaluate fitting stability and $K_S$ decay contamination, the lower fitting mass boundary is systematically varied from the nominal value 0.6 GeV/${\rm c^2}$ to 0.57 GeV/${\rm c^2}$ and 0.65 GeV/${\rm c^2}$.
The Drell-S${\rm \ddot{o}ding}$ mass-shape uncertainty is further estimated with an alternative parametrised experimental function used in HERA measurement~\cite{H1:2020lzc}
\begin{equation}
    \begin{aligned}
        A_{n r}=\frac{f_{n r}}{\left(m_{\pi \pi}^2-4 m_\pi^2+\Lambda_{n r}^2\right)^{\delta_{n r}}},
    \end{aligned}
\end{equation}
where $f_{n r}$, $\Lambda_{n r}$, and $\delta_{n r}$ are free parameters. While this approach enhances model flexibility, it introduces sensitivity to local minima during the fitting process.
Uncorrelated uncertainties are evaluated through variations in topological selection criteria and adjustments to the MC model in acceptance and efficiency extractions. Uncorrelated uncertainties are about 5\% for $\rho^0$ photoproduction and 8\% for Drell-S${\rm \ddot{o}ding}$. An external 10\% uncertainty in integrated luminosity determination and a 3\% per-track reconstruction uncertainty are included. 
All datasets exhibit statistical consistency within their combined uncertainties. The final results are derived from a weighted average, where the weights are determined by the quadrature sum of statistical uncertainties and uncorrelated systematic contributions,
%The results of each dataset are consistent within uncertainties and combined with the weight using the statistic uncertainties and uncorrelated systematic uncertainties.
\begin{equation}
    \begin{aligned}
        %&w_i = \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}/W,\\ \text{where} \ &W=\sum_i \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}.
        w_i = \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}/(\sum_i \frac{1}{\delta_{i,stat}^2+\delta_{i,sysuncorr}^2}).
    \end{aligned}
\end{equation}
The total systematic uncertainty is obtained by combining the uncorrelated and correlated uncertainties in quadrature.

%Fig.~\ref{fig:3} shows the differential cross section $d^2\sigma/dp_T^2dy$ for Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction with their ratio on the pair $p_T$ dependence. The Drell-S${\rm \ddot{o}ding}$ exhibit a sharper decreasing slope with $p_T$ increase and an obviously smaller $p_T$ for the diffractive dips which are related to the nucleus imaging. The ratio shows a significant bump which definitively demonstrate Drell-S${\rm \ddot{o}ding}$ process is softer than the $\rho^0$ production although they are both $\gamma A \rightarrow \pi^+\pi^-A$ processes. The results indicate the photon hadronic structure that the virtual $\pi^+\pi^-$ pair fluctuation concentrate more at lower photon energy region compared to virtual $\rho^0$.

% gpt improved:
Figure~\ref{fig:3} presents the differential cross-section $d^2\sigma/d|t| dy$ for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction, along with their ratio as a function of $|t|$. The $\rho^0$ results are consistent with the previous measurement~\cite{STAR:2017enh}.
%The Drell-S${\rm \ddot{o}ding}$ process exhibits a steeper decline with increasing $p_T$ compared to $\rho^0$ photoproduction, with a noticeably lower $p_T$ position for the diffractive minima, which are associated with nuclear imaging. 
Compared to $\rho^0$ photoproduction, the Drell-S${\rm \ddot{o}ding}$ process exhibits a steeper decline with increasing $|t|$ with its diffractive minima shifted to lower $|t|$, reflecting a softer production mechanism and differences in the underlying photon hadronic structure.
The measured ratio reveals a pronounced bump at low $|t|$, suggesting that the virtual $\pi^+\pi^-$ configuration is spatially broader than the $\rho^0$ state. Theoretical calculations do not reproduce this trend, possibly due to missing dipole-size effects that are not accounted for in the model.

Figure~\ref{fig:4} shows the azimuthal anisotropy, quantified by the second-order cosine modulation amplitude, ${\rm A_{2\Delta\phi}}$, for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction as functions of the pair transverse momentum $p_T$ (left) and the invariant mass $M_{\pi^+\pi^-}$ (right) within rapidity $|y|<0.9$. The amplitudes, ${\rm A_{2\Delta\phi}}$, are determined by performing invariant mass fits in distinct $\Delta\phi$ or $p_T$-vs-$\Delta\phi$ intervals. To ensure sufficient statistical precision for resolving subtle features in the mass distribution, the $p_T$ range is divided into three bins: $0 < p_T < 0.03~\mathrm{GeV}/c$, $0.03 < p_T < 0.05~\mathrm{GeV}/c$, and $0.05 < p_T < 0.1~\mathrm{GeV}/c$. The resulting differential cross section as a function of $\Delta\phi$ is then used to extract the $\cos(2\Delta\phi)$ modulation amplitude. The right panel illustrates the $M_{\pi^+\pi^-}$ dependence of ${\rm A_{2\Delta\phi}}$ integrated over the full $p_T$ range, $0 < p_T < 0.1~\mathrm{GeV}/c$.
%Fig.~\ref{fig:4} presents the azimuthal anisotropy quantified by the amplitude of the second order cosine modulation $A_{2\Delta\phi}$ for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction as functions of the pair transverse momentum $p_T$ (left) and the invariant mass $M_{\pi^+\pi^-}$ (right) for rapidity $|y|<0.9$. In order to measure the amplitudes $A_{2\Delta\phi}$, the mass fits are performed in different $\Delta\phi$ or $p_T-\Delta\phi$ intervals. The pair $p_T$ is divided into three bins as $0<p_T<0.03$ GeV/c, $0.03<p_T<0.05$ GeV/c and $0.05<p_T<0.1$ GeV/c for the differential mass fits in $p_T-\Delta\phi$ intervals. This is to guarantee enough statistics for a series of good fits to the subtle mass shape. Consequently, the obtained differential cross section as a function of $\Delta\phi$ is used to reconstruct the amplitude of $cos(2(\Delta\phi))$ modulation. The mass dependence of the amplitude $A_{2\Delta\phi}$ in an integrated pair transverse momentum $0<p_T<0.1$ GeV/c is presented in the right figure.

The ${\rm A_{2\Delta\phi}}$ of the Drell-S${\rm \ddot{o}ding}$ process exhibits a similar $p_T$ dependence with the $\rho^0$ photoproduction and an enhancement in transverse momentum in the range $0.05<p_T<0.1$ GeV/c. For exclusive $\pi^+\pi^-$ production, the yield in this $p_T$ intervals constitutes about half of the yield over $0<p_T<0.1$ GeV/c. The Drell-S${\rm \ddot{o}ding}$ is known to have a softer $p_T$ distribution compared to $\rho^0$ from Fig.~\ref{fig:3}. Notably, the measured ${\rm A_{2\Delta\phi}}$ as a function of $M_{\pi^+\pi^-}$ for the Drell-S${\rm \ddot{o}ding}$ in $0 < p_T < 0.1~\mathrm{GeV}/c$ is systematically higher than that for $\rho^0$ photoproduction. When integrated over $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$, the difference corresponds to a significance of $4.6\sigma$, evaluated including all statistical and systematic uncertainties. Specifically, ${\rm A_{2\Delta\phi}}$ values for $0 < p_T < 0.1~\mathrm{GeV}/c$, $|y| < 0.9$ and $0.6 < M_{\pi^+\pi^-} < 0.9~\mathrm{GeV}/c^2$ are measured as $0.2702 \pm 0.0024 \pm 0.0120$ (Drell-S${\rm \ddot{o}ding}$) and $0.2181 \pm 0.0022 \pm 0.0050$ ($\rho^0$ photoproduction). The first quoted errors are statistical uncertainties while the second are systematical uncertainties.


Furthermore, the $A_{2\Delta\phi}$ is found to have a relatively flat $M_{\pi^+\pi^-}$ dependence, suggesting minimal photon energy dependence in spin-interference. The predictions of the EPA-VMD and NRP model are also compared with the data and found to understimate $A_{2\Delta\phi}$ at lower transverse momentum, $0<p_T<0.05$ GeV/c. Based on the $A_{2\Delta\phi}$ measurement, specific contributions to the difference for the exclusive resonance and non-resonance produced entangled $\pi^+\pi^-$ pairs in cooperation with spin-interference can be studied. The results show no clear coherence lost in scattering with a nucleus and no clear destructive interference caused by the $\pi^+p$ and $\pi^-p$ scattering asymmetric amplitudes in the Drell-S${\rm \ddot{o}ding}$ process. %It is also indicated no significant wave function collapse caused by the $\rho^0$ decay

% Final conclusion generated by DS
In conclusion, we report the observation of spin-interference in the Drell-S${\rm \ddot{o}ding}$ process and the pair $p_T$ and $M$ dependence of the differential cross section for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction in Au+Au UPC at $\sqrt{s_{NN}}=200$ GeV at RHIC. A model-based Drell-S${\rm \ddot{o}ding}$ shape is employed to separate different processes involved in exclusive $\pi^+\pi^-$ production. 
%The Drell-S${\rm \ddot{o}ding}$ process is observed obviously softer from the pair $p_T$ spectrum compared to $\rho^0$ photoproduction. 
The observation of spin-interference effects demonstrates that the non-resonant $\pi^+\pi^-$ pairs are entangled in the Drell-S${\rm \ddot{o}ding}$ process. The amplitude, ${\rm A_{2\Delta\phi}}$, for the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction are found to have similar decreasing trends along the pair $p_T$. Compared to $\rho^0$, an enhancement is observed for the Drell-S${\rm \ddot{o}ding}$ process for pair $p_T$ in the range $0.05<p_T<0.1$ GeV/c. The measured ${\rm A_{2\Delta\phi}}$ for these processes is found to have no obvious pair mass $M_{\pi^+\pi^-}$ dependence, and the amplitude $A_{2\Delta\phi}$ for Drell-S${\rm \ddot{o}ding}$ is 4.6 $\sigma$ higher than for $\rho^0$ photoproduction among the observed mass regions. Moreover, the observed Drell-S${\rm \ddot{o}ding}$ $|t|$ spectrum is softer when compared to $\rho^0$ photoproduction. A comprehensive analysis of the measurements is reported through the comparison between resonant and non-resonant $\pi^+\pi^-$ photoproduction. These results advance the exploration of quantum interference phenomena in photon–nucleus interactions, providing a basis for future investigations in ultraperipheral heavy-ion collisions.

%The exclusive $\pi^+\pi^-$ production can be measured as a probe to the nuclear gluon density and nuclear geometry. From the comparison between the Drell-S${\rm \ddot{o}ding}$ process and $\rho^0$ photoproduction, the photon hadronic structure by fluctuation to ($\rho^0$ and $\pi^+\pi^-$) and production mechanism could be studied with its impact on imaging the nucleus. 


%Acknowledgement










\bibliography{reference}






